Discovering Attractive Products based on Influence Sets

Skyline queries have been widely used as a practical tool for multi-criteria decision analysis and for applications involving preference queries. For example, in a typical online retail application, skyline queries can help customers select the most interesting, among a pool of available, products. Recently, reverse skyline queries have been proposed, highlighting the manufacturer's perspective, i.e. how to determine the expected buyers of a given product. In this work we develop novel algorithms for two important classes of queries involving customer preferences. We first propose a novel algorithm, termed as RSA, for answering reverse skyline queries. We then introduce a new type of queries, namely the k-Most Attractive Candidates k-MAC query. In this type of queries, given a set of existing product specifications P, a set of customer preferences C and a set of new candidate products Q, the k-MAC query returns the set of k candidate products from Q that jointly maximizes the total number of expected buyers, measured as the cardinality of the union of individual reverse skyline sets (i.e., influence sets). Applying existing approaches to solve this problem would require calculating the reverse skyline set for each candidate, which is prohibitively expensive for large data sets. We, thus, propose a batched algorithm for this problem and compare its performance against a branch-and-bound variant that we devise. Both of these algorithms use in their core variants of our RSA algorithm. Our experimental study using both synthetic and real data sets demonstrates that our proposed algorithms outperform existing, or naive solutions to our studied classes of queries.

==> abstract.tex <==
\begin{abstract}
Skyline queries have been widely used as a practical tool for
multi-criteria decision analysis and for applications involving
preference queries. For example, in a typical online retail
application, skyline queries can help customers select the most
interesting, among a pool of available, products. Recently, reverse
skyline queries have been proposed, highlighting the manufacturer's
perspective, i.e. how to determine the expected buyers of a given
product. In this work we develop novel algorithms for two important
classes of queries involving customer preferences. We first propose a
novel algorithm, termed as \rsl, for answering reverse skyline
queries.\eat{ We demonstrate that our \rsl algorithm significantly
reduces both the I/O cost, as well as the computation cost, when
compared to the state-of-the-art reverse skyline algorithm \brs, while
at the same time being able to quickly report the first members of the
reverse skyline set.} We then introduce a new type of queries, namely
the $k$-Most Attractive Candidates (\kmp) query. In this type of
queries, given a set of existing product specifications $P$, a set of
customer preferences $C$ and a set of new candidate products $Q$, the
\kmp query returns the set of $k$ candidate products from $Q$ that
jointly maximizes the total number of expected buyers, measured as the
cardinality of the union of individual reverse skyline sets (i.e.,
\emph{influence sets}). Applying existing approaches to solve this
problem would require calculating the reverse skyline set for each
candidate, which is prohibitively expensive for large data sets. We,
thus, propose a batched algorithm for this problem and compare its
performance against a branch-and-bound variant that we devise. Both of
these algorithms use in their core variants of our \rsl algorithm. Our
experimental study using both synthetic and real data sets
demonstrates that our proposed algorithms outperform existing, or
naive solutions to our studied classes of queries. \eat{can achieve
significant benefits outperform (\emph{i}) our \rsl algorithm outperforms the
\brs algorithm, for the reverse skyline problem, in terms of I/O, CPU
cost and progressiveness of the output, and (\emph{ii}) our proposed batch
and branch-and-bound algorithms significantly outperform naive
approaches that process each candidate individually.}

\end{abstract} 

==> algs2.tex <==
\section{Reverse Skyline Processing for Multiple Query Points}
\label{sec:kmp_algs}

Solving the \kmp problem requires processing multiple candidates, in
order to first determine their influence sets. Subsequently, the
algorithm presented in Section~\ref{sec:greedy} can determine the
solution of the \kmp problem.

\begin{algorithm}[t]
\scriptsize
	\KwIn{$Q$ a set of candidates, $T_P$ R-tree on products, $T_C$ R-tree on customers}
    \SetKwInput{KwVar}{Variables}
    \KwVar{$E_P(q_i)$ set of active product entries for $q_i$, $E_C(q_i)$ set of active customer entries for $q_i$, $RSKY(q_i)$ reverse skylines for $q_i$, $SKY(q_i)$ midpoint skylines of $q_i$}
	\Begin
	{
        \ForEach{$q_i \in Q$}
        {
            \While{$E_C(q_i) \neq \varnothing$}
            {
                $\rsl(q_i, T_P, T_C, E_P, E_C, RSKY, SKY) \rightarrow RSKY(q_i)$\;
            }
        }
	}
\caption{Basic Algorithm}
\label{fig:basic}
\end{algorithm}

\stitle{A baseline solution.} A natural way to process multiple
candidates would be to apply either the \brs or the \rsl algorithm for
each candidate individually, as shown in Alg.~\ref{fig:basic}. We
will refer to these approaches as \emph{basic}. The \emph{basic}
algorithm is very inefficient in terms of I/O accesses, because it
requires accessing each entry $e_p$ or $e_c$ entry multiple times, as
each entry may appear in the corresponding priority queue of several
candidates. \eat{Moreover, as we will explain later in this section, the
\emph{basic} algorithm does not...}


\stitle{Our \brsl algorithm.} In order to eliminate the drawbacks of
the basic algorithm, we now introduce our \brsl algorithm, which
exploits I/O commonalities and offers shared processing among
candidates. \brsl utilizes in its core the \rsl algorithm that we
presented in Section~\ref{sec:rsl}.

A key requirement for the efficient execution of \brsl is the
grouping of candidates in such a way that the candidates have a high
probability of sharing multiple active entries in their $E_P$ and
$E_C$ sets. If this is somehow possible to achieve, then each of these
entries, when expanded at an iteration of its \rsl subcomponent, will
be read from disk just once, for all these entries. 

%Note that whenever a $e_p$ ($e_c$) entry is expanded, its children entries are inserted in the $E_P$ ($E_C$) sets of a corresponding candidate only if these children entries cannot be safely pruned based on the currently found skyline of the candidate. 

%Besides its apparent I/O benefits, such a grouping may also result in reduced CPU processing. In order to understand why this may happen, we need to consider that when... \textbf{{\large Exoume na pros8esoume kati edw??}} In cases when the candidates are grouped appropriately, \textbf{{\large Bla Bla}}.



\eat{ \brsl is based on the key observation that candidates that are
contiguous in the multidimensional space usually share a large number
of active entries. Therefore, if we process these candidates in
parallel we can avoid these redundant I/Os. Assume that $B$ candidates
fit in main memory, with $B \ll |Q|$.  }

It is important to note that we cannot safely assume that the sets of
active entries, along with all the necessary data structures that
\brsl utilizes for their efficient processing, fit in main
memory. Based on the memory capabilities of the hardware which
executes the \brsl algorithm, and worst case estimates of the amount
of customer and product entries in the sets of active entries, let us
assume that $B$ candidates (where $B \ll |Q|$) fit in main memory and
will be processed as a batch. Using worst case estimates does not have
a severe impact in the performance of \brsl since, as we explain
later in this section and demonstrate experimentally, it is desirable
to utilize fairly modest values (i.e., 10 to 20) for $B$. Larger
values may result in joint processing of dissimilar candidates, thus
incurring unnecessary processing cost.

Initially, \brsl partitions the candidate set into $\lceil|Q|/B\rceil$
batches based on a locality preserving hashing function, such as the
Hilbert space filling curve. Therefore, each batch tends to include
only candidates that are close to each other in the multidimensional
space. Then, a modified version of the \rsl algorithm, which handles
batch processing of candidates, is executed on each batch
(Alg.~\ref{alg:brsl}). The candidates in each batch are processed in a
round robin fashion (Line~5).

\brsl proceeds similar to \rsl, except that whenever an entry $e_x$ is
expanded, all local priority queues in which $e_x$ appears are
appropriately updated. Recall that, for each candidate, children nodes
are first checked with the candidate's currently found skyline set,
and with other children nodes, as we discussed in
Section~\ref{sec:rsl_alg}. Only those nodes that are not pruned are
pushed to the priority queue of the respective
candidate. Alg.~\ref{alg:batchExpand} details the pseudocode for batch
updating the priority queues of the batch.



%\textbf{Optimizations} ... buffers, pulling strategies inside the batch (roundrobin?)


\begin{algorithm}[t]
\scriptsize
	\KwIn{$Q$ a set of candidates, $T_P$ R-tree on products, $T_C$ R-tree on customers}
    \SetKwInput{KwVar}{Variables}
    \KwVar{$E_P(q_i)$ heap of active product entries for $q_i$, $E_C(q_i)$ set of active customer entries for $q_i$, $RSKY(q_i)$ reverse skylines for $q_i$, $SKY(q_i)$ midpoint skylines of $q_i$, $B_j$ batches with $|B_j| = B$}
	\Begin
	{
        partition $Q$ into $\lceil|Q|/B\rceil$ batches $\rightarrow B_j$\;
        \ForEach{$B_j$}
        {
            \While{($RSKY(q_i)$ for all $q_i \in B_j$ have not been found)}
            {
                selectCandidate $\rightarrow q_i$\;
                \If{$E_C(q_i) \neq \varnothing$}
                {
                    BRSA($q_i$, $B_j$, $T_P$, $T_C$, $E_P(q_i)$, $E_C(q_i)$, $RSKY(q_i)$, $SKY(q_i)$)\;
                }
            }
        }
	}
\caption{Batch-RSA}
\label{alg:brsl}
\end{algorithm}



\begin{algorithm}[t]
\scriptsize
	\KwIn{$B$ a set of candidates, $T_P$ R-tree on products, $T_C$ R-tree on customers, $E_P(q_i)$ heap of active product entries for $q_i$, $E_C(q_i)$ set of active customer entries for $q_i$, $RSKY(q_i)$ reverse skylines of $q_i$, $SKY(q_i)$ midpoint skylines of $q_i$}
	\KwOut{$RSKY(q_i)$ reverse skylines of $q_i$}
	\Begin
	{
        \While{$E_C \neq \varnothing$}
        {
            dominated := false\;
            $E_C(q).pop() \rightarrow e_c$\;
            \If{dominated($e_c$, $SKY(q_i))$}
            {
                dominated := true\;
                continue\;
            }
            \If{$e_c$ is a non-leaf entry}
            {
                %\ForAll{$e_{c_l}$ children of $e_c$}
%                {
%                    \If{(dominated($e_{c_l}$, $SKY(q))$ == false)}
%                    {
%                        $E_C(q).push(e_{c_l})$\;
%                    }
%                }
                 BatchExpand($e_c$, $B$, $SKY(q_i)$, $E_C(q_i)$, $T_C$)\;
            }
            \Else
            {
                \ForEach{$e_p \in E_P(q)$}
                {
                    $midpoint(e_p, q_i) \rightarrow m$\;
                    \If{$e_c$ is dominated by $m$}
                    {
                        \If{$e_p$ is a leaf entry}
                        {
                            \If{(dominated($m$, $SKY(q_i))$ == false)}
                            {
                                $SKY(q_i).push(m)$\;
                            }
                            dominated := true\;
                            break\;
                        }
                        \Else
                        {
                            %\If{dominated($e_p$, $SKY(q_i))$}
%                            {
%                                $E_P(q_i).remove(e_p)$\;
%                            }
%                            \Else
%                            {
                            BatchExpand($e_p$, $B$, $SKY(q)$, $E_p(q)$, $T_P$)\;
%                            }
                        }
                        $E_P(q_i).remove(e_p)$\;
                    }
                }
                \If{(dominated == false)}
                {
                    $RSKY(q_i).push(e_c)$\;
                }
            }
	   }
    \Return{$RSKY(q_i)$}\;
    }
\caption{BRSA}
\label{alg:batch_rsl}
\end{algorithm}


\begin{algorithm}[t]
\begin{scriptsize}
	\KwIn{$e_x$ a product or customer entry, $B$ a set of candidates, $SKY(q_i)$ currently found midpoint skyline set w.r.t to $q_i$, $E_x(q_i)$ priority queue on $e_x$, $T_x$ index on $e_x$}
    \KwOut{$E_x$}
	\SetKwInput{KwVar}{Variables}
	\KwVar{$L_i$ queues on children of $e_x$}
	\Begin
	{
        \ForEach{$q_i \in B$}
        {
            $L_i := \varnothing$\;
        }
        \ForEach{$e_{x_l}$ children of $e_x$}
        {
            \If{$e_x$ is a product entry}
            {
                \ForEach{$q_i \in B$}
                {
                    \If{(dominated($e_{x_l}$, $L_i$) == true)}
                    {
                        continue;
                    }
                }
            }
            \ForEach{$q_i \in B$}
            {
                \If{(dominated($e_{x_l}$, $SKY(q_i)$) == false)}
                {
                    $L_i.push(e_{x_l})$\;
                }
            }
        }
        \ForEach{$q_i \in B$}
        {
            \ForEach{$e_{x_l} \in L_i$}
            {
                $E_x(q_i).push(e_{x_l})$\;
            }
        }
        \Return{$E_x$}\;
    }
\caption{BatchExpand}
\label{alg:batchExpand}
\end{scriptsize}
\end{algorithm}



==> conclusion.tex <==
\section{Conclusions}
\label{sec:conclusion}

In this work, we studied two important class of queries involving
customer preferences. We first proposed a novel algorithm, \rsl, for
reverse skyline query evaluation. We then introduced a new type of
skyline query, termed as the $k$-Most Attractive Candidates (\kmp)
query; \kmp selects the set of $k$ candidate products that jointly
maximizes the total number of expected buyers. We propose a batch
algorithm, which utilizes in its core our \rsl algorithm, but
significantly improves upon naive techniques that process all
candidate products individually, for answering \kmp queries. Our
extensive experimental study on both real and synthetic data sets
demonstrates that (\emph{i}) \rsl outperforms the \brs algorithm, for the
reverse skyline problem, in terms of I/O, CPU cost and progressiveness
of output, and (\emph{ii}) that our proposed batch algorithm outperforms
branch-and-bound and baseline approaches for the \kmp query.




==> exps.tex <==
\section{Experimental Evaluation}
\label{sec:exps}


We now evaluate the performance of our proposed methods using both
real and synthetically generated data. All algorithms examined in our
experiments were implemented in C++\eat{, compiled with gcc} and
executed on a 3GHz Intel Core 2 Duo CPU with 4GB RAM running Debian
Linux. The code for the \brs algorithm was provided to us by the
authors of~\cite{WTW+09}.

\subsection{Used Data Sets} \label{sec:setup}
We used a publicly available generator \cite{Rand} in order to
construct synthetic data sets. We distinguish three classes of data
sets, based on the distribution of the attributes' values. In uniform
(UN) data sets, attribute values are drawn from a uniformly random
distribution. In anti-correlated (AC) data sets, points having
desirable attribute values in one dimension are more likely to have
less desirable values in the other dimensions (e.g., laptops with
faster CPU are more likely to be more expensive). Finally, in
correlated (CO) data sets, points with desirable attribute values in
one dimension tend to have good values in other dimensions as
well. 
%Results involving CO data can be found in the full version of this paper (available at: http://www.softnet.tuc.gr/~adeli/TR-MAC.pdf).

\eat{The clustered dataset, namely (CL), models the case when multiple
users share similar preferences, or several products have similar
specifications. For CL, first $N_C$ cluster centroids are selected
randomly from a uniform distribution. Then, for each cluster we
assigned $|P|/N_C$ points. The coordinate for each point follows a
gaussian distribution, with mean equal to the attribute value of the
corresponding centroid and variance $\sigma = 1$. For all
distributions, the size of each domain was set to 10000.  }

We also compared our algorithms on two real world data sets. The NBA
data set (NBA) consists of 17,265 5-dimensional points, representing a
player's annual performance. The dimensions are average values for the
number of points scored, rebounds, assists, steals and blocks. The
household data set (HOUSE), consists of 127,930 6-dimensional points,
representing the percentage of an American family's annual income
spent on 6 types of expenditure: gas, electricity, water, heating,
insurance, and property tax. We used the real data sets as products
(NBA-P and HOUSE-P resp.). Both data sets were normalized to have a
range [0,1000] on each dimension. In order to construct customer
(NBA-C, HOUSE-C) and candidate sets (NBA-Q, HOUSE-Q), for each point
in NBA-P (HOUSE-P resp.) we added a gaussian noise with mean equal to
the value of the actual point for the respective dimension and
variance equal to 5 and 10 respectively. For each data set, we built
an R-tree with a page size of 4K.



\subsection{Algorithms Used}
We compared the performance of the \brs algorithm with our \rsl
algorithm and our \brsl algorithm for computing the answer to \kmp
queries. Please recall that neither \brs nor \rsl perform any batching
of the examined candidates, while \brsl presorts the new candidate
products (candidates) and assigns them to partitions (batches).

\begin{algorithm}[t]
\scriptsize
	\KwIn{$Q$ a set of candidates, $T_P$ R-tree on products, $T_C$ aR-tree on customers, $k$}
	\KwOut{$Q_k$ min-heap on $\is^+$ containing the most attractive candidates, $|Q_k| = k$}
	\SetKwInput{KwVar}{Variables}
	\KwVar{$E_P(q_i)$ heap of active product entries for $q_i$, $E_C(q_i)$ heap of active customer entries for $q_i$, $RSKY(q_i)$ reverse skylines for $q_i$, $SKY(q_i)$ midpoint skylines of $q_i$, $\is^+(q_i)$ upper bound for $\is(q_i)$, $H_{max}$ max-heap on $\is^+$, $\is(Q_k)$ current lower bound of joint influence score}
	\Begin
	{
        $Q_k := \varnothing $\;
        \ForEach{$q_i \in Q$}
        {
            $\rsl(q_i) := \varnothing $; $\is^+(q_i) := |C|$;
            $E_P(q_i) := \varnothing $; $E_C(q_i) := \varnothing $\;
        }
        \While{$Q \neq \varnothing$}
        {
            $H_{max}.pop() \rightarrow q_i$\;
	    \tcc{Process $q_i$ if $\is(q_i)$ not completely refined}
            \If{$E_C(q_i) \neq \varnothing$}
            {
	
                B\rsl($q_i$, $T_P$, $T_C$, $E_P$, $E_C$, $RSKY$, $SKY$, $\is^+$, $\is^-$)\;
                \ForEach{$q_i \in Q$}
		{
		  \tcc{Run $\kgcs$ using $\is^-$ for each candidate, to get $\is^-(Q_k)$}

                  $\kgcs \rightarrow Q^-_k$\;

		  \tcc{Run $\kgcs$ using $\is^+$ for each candidate, to
		  get $\is^+(Q_{k-1})$. Force $\kgcs$ to start by selecting
		  $q_i$.}
		    $\kgcs \rightarrow Q_{k-1}$\;

                    \If{$\is^+(q_i) + \is^+(Q_{k-1}) < \is^-(Q_k)$}
                    {
                        $Q := Q - \{q_i\}$; \CommentSty{//Prune $q_i$}
                    }
                }
            }
        }
        \Return{$Q$}\;
	}
\caption{\bbkmp}
\label{alg:bbkmp}
\end{algorithm}



In order to add another interesting baseline solution against \rsl and
\brsl, we also devised and implemented a branch-and-bound algorithm,
presented in Alg.~\ref{alg:bbkmp}, for the \kmp problem. The \bbkmp
maintains for each candidate, apart from its influence set, the
currently found upper bound of its influence score. \bbkmp associates
with each $q \in Q$ an R-tree $T_P(q)$ on the products and an
aggregate (count) aR-tree ~\cite{PKZT01} $T^A_C(q)$ on the
customers. The aR-tree maintains ${e_c}.count$, i.e. the number of
leaf entries that lie within the subtree of ${e_c}$, for each node
$e_c$. To understand the use of the aR-tree, consider the case when a
$e_c$ entry can be pruned. With a regular R-tree on the customers, we
would have to access the pruned entry and enumerate the customer
points that lie within $e_c$'s subtree in order to update the upper
bound of the influence score. With an aR-tree this step can be
avoided.



\bbkmp proceeds in iterations and is executed similar to
\bbrs with one main exception. If a customers' entry $e_c$ can be pruned,
\bbkmp does not access $e_c$; instead the aggregate information ${e_c}.count$
is subtracted from $\is^+(q)$. Further, %instead of executing the \brsl algorithm for each candidate $q$ until $E_C(q)$ becomes empty,
\bbkmp picks one
candidate at a time (Line~6), performs a single execution of \brsl
(Line~8) and updates $\is^+(q)$. In each iteration, \bbkmp selects to
examine the candidate $q_i$ with the highest current $\is^+(q_i)$, and
processes the candidate, unless the candidate is completely refined
(Line~7). Finally, \bbkmp prunes $q_i$ based on the following pruning
rule: Let $\is^-(Q_k)$ denote the lower bound of the currently optimal solution
based on Alg.~\ref{alg:kGCS}. Let $\is^+(Q_{k-1})$ denote the
upper bound of the optimal solution based on Alg.~\ref{alg:kGCS},
when forcing the algorithm to include $q_i$ in the solution. If the condition in
Line~12 of \bbkmp is satisfied, then $q_i$ can safely be pruned, even
if its exact influence set has not been determined.

The \bbkmp algorithm is introduced and compared against, since a
branch and bound technique seems natural for the \kmp
problem. However, it has several drawbacks. First, \bbkmp cannot
partition the candidates in batches, unless it aims to solve the
\gkmp{1} problem. To understand why this is the case, let us consider
the following scenario of seeking the solution to \gkmp{2}. Let us
assume a candidate $q_i: |RSKY(q_i)|=1$, and that the customer that
$q_i$ has in its reverse skyline does not appear in the skyline of any
other node. Then, it is not hard to devise cases where the solution to
\gkmp{2} may involve combining $q_i$ with another candidate $q_j$ that
has the largest influence score. Thus, if we want to enable \bbkmp to
perform pruning, then all candidates need to be processed in a single
batch. However, with this setup, the performance of \bbkmp was
disappointing (this point will be made clear when we also examine the
performance of \brsl when using very large batch sizes).


We thus only present experiments for the \gkmp{1} case. This scenario
is a best case scenario for the \bbkmp algorithm, since it allows its
implementation using batching of the candidates (similarly to \brsl)
and also allows the pruning of candidates. It is important to
emphasize that the \brs, the \rsl and the \brsl algorithms are not
influenced by the value of $k$, since they first determine the
influence sets of all candidates, and then run
Alg.~\ref{alg:kGCS} (which requires a few milliseconds to run) to
produce the final solution.




\eat{
\begin{table}[h!]
\centering
\begin{small}
\begin{tabular}[b]{| @{\hspace{0.05in}} c @{\hspace{0.05in}} | @{\hspace{0.05in}} c @{\hspace{0.05in}} | @{\hspace{0.05in}} c @{\hspace{0.05in}} | }
\hline
\textbf{Algorithm}& \textbf{Acronym} & \textbf{Section} \\ \hline
\brs & \brs & \ref{sec:brs} \\ \hline
\rsl & \rsl & \ref{sec:rsl_alg} \\ \hline
%Batch-\brs & \bbrs & \ref{sec:kmp_algs} \\ \hline
Batch-\rsl & B-\rsl & \ref{sec:kmp_algs} \\ \hline
%Branch-and-Bound BRS & BB-BRS & \ref{sec:bbkmp} \\ \hline
Branch-and-Bound \rsl & BB-\rsl & \ref{sec:bbkmp} \\ \hline
\end{tabular}
\end{small}
\caption{Algorithms in examination} \centering
\label{tab:algos}
\end{table}
}

\subsection{Metrics and Default Parameter Setting}

In each experimental setup, we vary a single parameter while setting
the remaining to their default values. Table~\ref{tab:params}
summarizes the parameters under investigation and their corresponding
ranges; the default values are depicted in bold.

\begin{table}[h!]
\caption{Parameters and values} \centering
\label{tab:params}
\centering
\begin{small}
\begin{tabular}[b]{| @{\hspace{0.05in}} c @{\hspace{0.05in}} | @{\hspace{0.05in}} c @{\hspace{0.05in}} |}
\hline
\textbf{Parameter}& \textbf{Range}\\ \hline
P dataset cardinality ($|P|$) & 10K, \textbf{100K}, 1M, 5M \\ \hline
C dataset cardinality ($|C|$) & 10K, \textbf{100K}, 1M, 5M \\ \hline
Q dataset cardinality ($|Q|$) & 100, \textbf{1K}, 10K \\ \hline
Dimensionality ($D$) & 2, \textbf{3}, 4, 5 \\ \hline
Batch Size ($|B|$)& 5, \textbf{10}, 20, 50, 100 \\ \hline
%Buffer Size & 50, \textbf{100}, 500 \\ \hline
%k ($k$) & 1, \textbf{3}, 10, 20, 50 \\ \hline
\end{tabular}
\end{small}
\end{table}




Each set of experiments examines the performance of all methods in
\kmp query evaluation.\eat{ with respect to the parameter currently in
investigation.} In particular, we measure (\emph{i}) the number of I/O
operations (either on product or on customer entries), and (\emph{ii}) the
actual query processing time, consisting of the time spent both on
CPU, as well as the time spent on I/O operations. Recall that single
point skyline and batch algorithms require an additional step that
greedily selects the best candidates after identifying the influence
set of each candidate. However, the processing time required for this
step is negligible (a few milliseconds) using Alg.~\ref{alg:kGCS}
compared to the time required for the algorithm execution. Please note
that the experimental results for the \brs and the \rsl algorithms can
also be used for evaluating their performance in single point reverse
skyline query processing, since these algorithms simply process each
candidate one after the other. Essentially, for both \brs and \rsl
algorithms, the plots represent the total CPU time and I/O operations
required for processing a workload of $|Q|$ reverse skyline queries.


\subsection{Experimental Results}
\label{sec:results}




\stitle{Sensitivity Analysis vs. $|P|$}. We first performed a
sensitivity analysis with respect to the size of the product data
set. As depicted in
Figures~\ref{plt:aCPUvsPstacked}-\ref{plt:cCPUvsPstacked}, in terms of
CPU cost, \rsl is notably more efficient than \brs, particularly as
the size of $|P|$ grows large. For instance, for uniformly distributed
data with $|P| = 5M$ (Fig.~\ref{plt:cCPUvsPstacked}), \brs entails
$\sim$8 times larger processing cost than \rsl. With respect to the
total I/Os required
(Figures~\ref{plt:aIOvsPstacked}-\ref{plt:cIOvsPstacked}), \rsl
exhibits equivalent performance with \brs in the case where product
and customer data have the same size (100K both). However, as the size
of products increases, the I/Os required by \rsl are significantly
fewer than those of \brs. Notice the different behavior of the two
algorithms with respect to the type of I/Os; \brs performs fewer
accesses on the product index, whereas \rsl is more efficient on
customer I/Os. This is expected since the two algorithms follow
different visiting orders. However, as demonstrated in this set of
experiments, the strategy followed by \rsl is more efficient in terms
of the total number of I/Os. Further, both batch and branch-and-bound
extensions of \rsl achieve significant performance gains in all
settings. Essentially they remain largely unaffected by the size of
$|P|$. \bbkmp is slightly more expensive than \brsl, since it requires
more index space for the same size of input in order to maintain the
aggregate information, and hence it entails more I/Os than \brsl on
the customer index.

\eat{
\begin{figure}[t]
\centering
\subfigure[CPU cost vs. $|P|$ (AC)]{
\includegraphics[width=1.62in]{a_CPU_P_stacked}
\label{plt:aCPUvsPstacked}
}
\subfigure[CPU cost vs. $|P|$ (UN)]{
\includegraphics[width=1.62in]{i_CPU_P_stacked}
\label{plt:iCPUvsPstacked}
}
\eat{
\subfigure[CPU cost vs. $|P|$ (CO)]{
\includegraphics[width=0.31\textwidth]{c_CPU_P_stacked}
\label{plt:cCPUvsPstacked}
}
}
\subfigure[I/Os vs. $|P|$ (AC)]{
\includegraphics[width=1.62in]{a_IO_P_stacked}
\label{plt:aIOvsPstacked}
}
\subfigure[I/Os vs. $|P|$ (UN)]{
\includegraphics[width=1.62in]{i_IO_P_stacked}
\label{plt:iIOvsPstacked}
}
\eat{
\subfigure[I/Os vs. $|P|$ (CO)]{
\includegraphics[width=0.31\textwidth]{c_IO_P_stacked}
\label{plt:cIOvsPstacked}
}
}
\caption{Varying number of products $|P|$} \centering
\label{fig:exps_P}
\end{figure}
}

\begin{figure*}[t]
\centering
\subfigure[CPU cost vs. $|P|$ (AC)]{
\includegraphics[width=0.31\textwidth]{a_CPU_P_stacked}
\label{plt:aCPUvsPstacked}
}
\subfigure[CPU cost vs. $|P|$ (UN)]{
\includegraphics[width=0.31\textwidth]{i_CPU_P_stacked}
\label{plt:iCPUvsPstacked}
}
\subfigure[CPU cost vs. $|P|$ (CO)]{
\includegraphics[width=0.31\textwidth]{c_CPU_P_stacked}
\label{plt:cCPUvsPstacked}
}
\subfigure[I/Os vs. $|P|$ (AC)]{
\includegraphics[width=0.31\textwidth]{a_IO_P_stacked}
\label{plt:aIOvsPstacked}
}
\subfigure[I/Os vs. $|P|$ (UN)]{
\includegraphics[width=0.31\textwidth]{i_IO_P_stacked}
\label{plt:iIOvsPstacked}
}
\subfigure[I/Os vs. $|P|$ (CO)]{
\includegraphics[width=0.31\textwidth]{c_IO_P_stacked}
\label{plt:cIOvsPstacked}
}
\caption{Varying number of products $|P|$} \centering
\label{fig:exps_P}
\end{figure*}





\stitle{Sensitivity Analysis vs. $|C|$}. Next, we compared the
efficiency of our algorithms with respect to the size of the customer
data set. Figures~\ref{plt:aCPUvsCstacked}-\ref{plt:cCPUvsCstacked}
depict the CPU cost, while
Figures~\ref{plt:aIOvsCstacked}-\ref{plt:cIOvsCstacked} plot the I/O
cost. As illustrated, \rsl is slightly more efficient in terms of the
CPU spent, whereas \rsl and \brs require roughly the same number of
I/Os. To justify this behavior, recall that \rsl processes customers
in iterations, hence the number of iterations grows with $|C|$. In
contrast, in each iteration of \brs multiple $e_c$ entries might be
processed. However, even in this (worst case for \rsl) experimental
setup, \rsl performs equivalently to the \brs algorithm. Finally, for
\kmp queries both \brsl and \bbkmp algorithms are significantly more
efficient from the single point algorithms.

\eat{
\begin{figure}[t]
\centering
\subfigure[CPU cost vs. $|C|$ (AC)]{
\includegraphics[width=1.62in]{a_CPU_C_stacked}
\label{plt:aCPUvsCstacked}
}
\subfigure[CPU cost vs. $|C|$ (UN)]{
\includegraphics[width=1.62in]{i_CPU_C_stacked}
\label{plt:iCPUvsCstacked}
}
\eat{
\subfigure[CPU cost vs. $|C|$ (CO)]{
\includegraphics[width=0.31\textwidth]{c_CPU_C_stacked}
\label{plt:cCPUvsCstacked}
}
}
\subfigure[I/Os vs. $|C|$ (AC)]{
\includegraphics[width=1.62in]{a_IO_C_stacked}
\label{plt:aIOvsCstacked}
}
\subfigure[I/Os vs. $|C|$ (UN)]{
\includegraphics[width=1.62in]{i_IO_C_stacked}
\label{plt:iIOvsCstacked}
}
\eat{
\subfigure[I/Os vs. $|C|$ (CO)]{
\includegraphics[width=0.31\textwidth]{c_IO_C_stacked}
\label{plt:cIOvsCstacked}
}
}
\caption{Varying number of customers $|C|$} \centering
\label{fig:exps_C}
\end{figure}
}

\begin{figure*}[t]
\centering
\subfigure[CPU cost vs. $|C|$ (AC)]{
\includegraphics[width=0.31\textwidth]{a_CPU_C_stacked}
\label{plt:aCPUvsCstacked}
}
\subfigure[CPU cost vs. $|C|$ (UN)]{
\includegraphics[width=0.31\textwidth]{i_CPU_C_stacked}
\label{plt:iCPUvsCstacked}
}
\subfigure[CPU cost vs. $|C|$ (CO)]{
\includegraphics[width=0.31\textwidth]{c_CPU_C_stacked}
\label{plt:cCPUvsCstacked}
}
\subfigure[I/Os vs. $|C|$ (AC)]{
\includegraphics[width=0.31\textwidth]{a_IO_C_stacked}
\label{plt:aIOvsCstacked}
}
\subfigure[I/Os vs. $|C|$ (UN)]{
\includegraphics[width=0.31\textwidth]{i_IO_C_stacked}
\label{plt:iIOvsCstacked}
}
\subfigure[I/Os vs. $|C|$ (CO)]{
\includegraphics[width=0.31\textwidth]{c_IO_C_stacked}
\label{plt:cIOvsCstacked}
}
\caption{Varying number of customers $|C|$} \centering
\label{fig:exps_C}
\end{figure*}


\stitle{Sensitivity Analysis vs. $|Q|$}. We now investigate the
performance of all algorithms in evaluating \kmp queries with respect
to the size of the candidates data
set. Figures~\ref{plt:aCPUvsQstacked}-\ref{plt:cIOvsQstacked} plot the
results in logarithmic scale. Recall that for both \brs and \rsl plots
represent the total time (I/Os resp.) required for a workload of $|Q|$
reverse skyline queries, which are processed one after the other,
whereas \brsl and \bbkmp proceed in batches. An interesting
observation comes when analyzing the CPU cost of \brsl and \bbkmp in
comparison to single point algorithms. \brsl and \bbkmp both require
more CPU cost than \rsl, because of the time spent on maintaining
priority queues for all candidates in the batch. However, their total
processing cost is less because of the reduced number of required
I/Os. Overall, \brsl is the most efficient and scalable algorithm for
the \kmp query when the size of $|Q|$ increases.

\eat{
\begin{figure}[t]
\centering
\subfigure[CPU cost vs. $|Q|$ (AC)]{
\includegraphics[width=1.62in]{a_CPU_Q_stacked}
\label{plt:aCPUvsQstacked}
}
\subfigure[CPU cost vs. $|Q|$ (UN)]{
\includegraphics[width=1.62in]{i_CPU_Q_stacked}
\label{plt:iCPUvsQstacked}
}
\eat{
\subfigure[CPU cost vs. $|Q|$ (CO)]{
\includegraphics[width=0.31\textwidth]{c_CPU_Q_stacked}
\label{plt:cCPUvsQstacked}
}
}
\subfigure[I/Os vs. $|Q|$ (AC)]{
\includegraphics[width=1.62in]{a_IO_Q_stacked}
\label{plt:aIOvsQstacked}
}
\subfigure[I/Os vs. $|Q|$ (UN)]{
\includegraphics[width=1.62in]{i_IO_Q_stacked}
\label{plt:iIOvsQstacked}
}
\eat{
\subfigure[I/Os vs. $|Q|$ (CO)]{
\includegraphics[width=0.31\textwidth]{c_IO_Q_stacked}
\label{plt:cIOvsQstacked}
}
}
\caption{Varying number of candidates $|Q|$} \centering
\label{fig:exps_Q}
\end{figure}
}

\begin{figure*}[t]
\centering
\subfigure[CPU cost vs. $|Q|$ (AC)]{
\includegraphics[width=0.31\textwidth]{a_CPU_Q_stacked}
\label{plt:aCPUvsQstacked}
}
\subfigure[CPU cost vs. $|Q|$ (UN)]{
\includegraphics[width=0.31\textwidth]{i_CPU_Q_stacked}
\label{plt:iCPUvsQstacked}
}
\subfigure[CPU cost vs. $|Q|$ (CO)]{
\includegraphics[width=0.31\textwidth]{c_CPU_Q_stacked}
\label{plt:cCPUvsQstacked}
}
\subfigure[I/Os vs. $|Q|$ (AC)]{
\includegraphics[width=0.31\textwidth]{a_IO_Q_stacked}
\label{plt:aIOvsQstacked}
}
\subfigure[I/Os vs. $|Q|$ (UN)]{
\includegraphics[width=0.31\textwidth]{i_IO_Q_stacked}
\label{plt:iIOvsQstacked}
}
\subfigure[I/Os vs. $|Q|$ (CO)]{
\includegraphics[width=0.31\textwidth]{c_IO_Q_stacked}
\label{plt:cIOvsQstacked}
}
\caption{Varying number of candidates $|Q|$} \centering
\label{fig:exps_Q}
\end{figure*}


\stitle{Sensitivity Analysis vs. $D$}. Next, we varied the
dimensionality of the data sets from 2 to 5 and investigated the
performance of all algorithms with respect to
$D$. Figures~\ref{plt:aCPUvsDstacked}-\ref{plt:cCPUvsDstacked} and
\ref{plt:aIOvsDstacked}-\ref{plt:cIOvsDstacked} plot the results for
the CPU and I/O costs respectively. As expected (refer to the
complexity analysis in Section~\ref{sec:shortcomings}), in higher
dimensional data \brs requires one order of magnitude more processing
time to complete than \rsl. Clearly, as shown in
Figures~\ref{plt:aCPUvsDstacked}-\ref{plt:cCPUvsDstacked}, in higher
dimensions the I/O cost of \brs is dominated by the processing cost
(notice that plots are in logarithmic scale). To understand this,
recall that each dominance check requires $D$ comparisons, and that
the number of minmax points per entry is $D$.

\eat{
\begin{figure}[t]
\centering
\subfigure[CPU cost vs. $D$ (AC)]{
\includegraphics[width=1.62in]{a_CPU_DIM_stacked}
\label{plt:aCPUvsDstacked}
}
\subfigure[CPU cost vs. $D$ (UN)]{
\includegraphics[width=1.62in]{i_CPU_DIM_stacked}
\label{plt:iCPUvsDstacked}
}
\eat{
\subfigure[CPU cost vs. $D$ (CO)]{
\includegraphics[width=0.21\textwidth]{c_CPU_DIM_stacked}
\label{plt:cCPUvsDstacked}
}
}
\subfigure[I/Os vs. $D$ (AC)]{
\includegraphics[width=1.62in]{a_IO_DIM_stacked}
\label{plt:aIOvsDstacked}
}
\subfigure[I/Os vs. $D$ (UN)]{
\includegraphics[width=1.62in]{i_IO_DIM_stacked}
\label{plt:iIOvsDstacked}
}
\eat{
\subfigure[I/Os vs. $D$ (CO)]{
\includegraphics[width=0.21\textwidth]{c_IO_DIM_stacked}
\label{plt:cIOvsDstacked}
}
}
\caption{Varying number of dimensions $D$} \centering
\label{fig:exps_D}
\end{figure}
}

\begin{figure*}[t]
\centering
\subfigure[CPU cost vs. $D$ (AC)]{
\includegraphics[width=0.31\textwidth]{a_CPU_DIM_stacked}
\label{plt:aCPUvsDstacked}
}
\subfigure[CPU cost vs. $D$ (UN)]{
\includegraphics[width=0.31\textwidth]{i_CPU_DIM_stacked}
\label{plt:iCPUvsDstacked}
}
\subfigure[CPU cost vs. $D$ (CO)]{
\includegraphics[width=0.31\textwidth]{c_CPU_DIM_stacked}
\label{plt:cCPUvsDstacked}
}
\subfigure[I/Os vs. $D$ (AC)]{
\includegraphics[width=0.31\textwidth]{a_IO_DIM_stacked}
\label{plt:aIOvsDstacked}
}
\subfigure[I/Os vs. $D$ (UN)]{
\includegraphics[width=0.31\textwidth]{i_IO_DIM_stacked}
\label{plt:iIOvsDstacked}
}
\subfigure[I/Os vs. $D$ (CO)]{
\includegraphics[width=0.31\textwidth]{c_IO_DIM_stacked}
\label{plt:cIOvsDstacked}
}
\caption{Varying number of dimensions $D$} \centering
\label{fig:exps_D}
\end{figure*}


\stitle{Sensitivity Analysis vs. $|B|$}. We now examine the batch and
branch-and-bound algorithms in respect to the batch size $|B|$. Recall
that each candidate is hashed to the appropriate batch, such that each
batch contains only candidates that are close in the initial
space. Therefore, we expect that candidates in the same batch will
share pruning of product or customer entries. We set each batch to
contain from 5 to 100 candidates and plotted the results in
Figures~\ref{plt:aCPUvsBATCHstacked}-\ref{plt:cIOvsBATCHstacked}. As
depicted, as batch size increases, the total I/O operations fall since
more pruning can be shared among candidates. However, the total
processing cost grows rapidly. This happens due to the following
reason. When the batch size is larger, candidates belonging to the
batch are dissimilar, and hence they will not benefit from the
expansion of entries from other candidates. Rather, children entries
have to be pushed into the local priority queues of most of the
candidates. This results to: (\emph{i}) increasing cost and larger space
required for the maintenance of $E_P(q_i)$ and $E_C(q_i)$, and (\emph{ii})
more processing time for subsequent dominance checks. As showcased by
the experiments, keeping smaller batch sizes (up to 10 candidates)
positively favors the performance of both \brsl and \bbkmp. At this
point it is important to emphasize that keeping all candidates in a
single batch is impractical; this fact restrains \bbkmp algorithm for
being used for \kmp queries other than $\gkmp{1}$.

\eat{
\begin{figure}[t]
\centering
\subfigure[CPU cost vs. $|B|$ (AC)]{
\includegraphics[width=0.21\textwidth]{a_CPU_BATCH_stacked}
\label{plt:aCPUvsBATCHstacked}
}
\subfigure[CPU cost vs. $|B|$ (UN)]{
\includegraphics[width=0.21\textwidth]{i_CPU_BATCH_stacked}
\label{plt:iCPUvsBATCHstacked}
}
\eat{
\subfigure[CPU cost vs. $|B|$ (CO)]{
\includegraphics[width=0.23\textwidth]{c_CPU_BATCH_stacked}
\label{plt:cCPUvsBATCHstacked}
}
}
\subfigure[I/Os vs. $|B|$ (AC)]{
\includegraphics[width=0.21\textwidth]{a_IO_BATCH_stacked}
\label{plt:aIOLvsBATCHstacked}
}
\subfigure[I/Os vs. $|B|$ (UN)]{
\includegraphics[width=0.21\textwidth]{i_IO_BATCH_stacked}
\label{plt:iIOvsBATCHstacked}
}
\eat{
\subfigure[I/Os vs. $|B|$ (CO)]{
\includegraphics[width=0.23\textwidth]{c_IO_BATCH_stacked}
\label{plt:cIOvsBATCHstacked}
}
}
\caption{Varying batch size $|B|$} \centering
\label{fig:exps_batch}
\end{figure}
}

\begin{figure*}[t]
\centering
\subfigure[CPU cost vs. $|B|$ (AC)]{
\includegraphics[width=0.31\textwidth]{a_CPU_BATCH_stacked}
\label{plt:aCPUvsBATCHstacked}
}
\subfigure[CPU cost vs. $|B|$ (UN)]{
\includegraphics[width=0.31\textwidth]{i_CPU_BATCH_stacked}
\label{plt:iCPUvsBATCHstacked}
}
\subfigure[CPU cost vs. $|B|$ (CO)]{
\includegraphics[width=0.31\textwidth]{c_CPU_BATCH_stacked}
\label{plt:cCPUvsBATCHstacked}
}
\subfigure[I/Os vs. $|B|$ (AC)]{
\includegraphics[width=0.31\textwidth]{a_IO_BATCH_stacked}
\label{plt:aIOLvsBATCHstacked}
}
\subfigure[I/Os vs. $|B|$ (UN)]{
\includegraphics[width=0.31\textwidth]{i_IO_BATCH_stacked}
\label{plt:iIOvsBATCHstacked}
}
\subfigure[I/Os vs. $|B|$ (CO)]{
\includegraphics[width=0.31\textwidth]{c_IO_BATCH_stacked}
\label{plt:cIOvsBATCHstacked}
}
\caption{Varying batch size $|B|$} \centering
\label{fig:exps_batch}
\end{figure*}


%\stitle{Sensitivity Analysis vs. buffer size}.
%
%\begin{figure*}[t]
%\centering
%\subfigure[I/Os vs. buffer size (AC)]{
%\includegraphics[width=0.31\textwidth]{a_B_IO_BUFFER_stacked}
%\label{plt:aIOvsBUFFERstacked}
%}
%\subfigure[I/Os vs. buffer size (UN)]{
%\includegraphics[width=0.31\textwidth]{i_B_IO_BUFFER_stacked}
%\label{plt:iIOvsBUFFERstacked}
%}
%\subfigure[I/Os vs. buffer size (CO)]{
%\includegraphics[width=0.31\textwidth]{c_B_IO_BUFFER_stacked}
%\label{plt:cOPvsBUFFERstacked}
%}
%\caption{Varying buffer size} \centering
%\label{fig:exps_buffer}
%\end{figure*}


%\stitle{Sensitivity Analysis vs $k$}.
%
%\begin{figure}[h!]
%\centering
%\subfigure[CPU cost vs. $k$ (UN)]{
%\hspace{-0.15in}
%\includegraphics[width=0.49\columnwidth]{i_CPU_KAPA_stacked}
%\label{plt:CPUvsKstacked}
%}
%\subfigure[I/Os vs. $k$ (UN)]{
%\hspace{-0.15in}
%\includegraphics[width=0.49\columnwidth]{i_IO_KAPA_stacked}
%\label{plt:iIOvsKRstacked}
%}
%\subfigure[CPU cost vs. $k$ (AC)]{
%\hspace{-0.15in}
%\includegraphics[width=0.49\columnwidth]{a_CPU_KAPA_stacked}
%\label{plt:aCPUvsKstacked}
%}
%\subfigure[I/Os vs. $k$ (AC)]{
%\hspace{-0.15in}
%\includegraphics[width=0.49\columnwidth]{a_IO_KAPA_stacked}
%\label{plt:aIOvsKstacked}
%}
%\subfigure[CPU cost vs. $k$ (CO)]{
%\hspace{-0.15in}
%\includegraphics[width=0.49\columnwidth]{c_CPU_KAPA_stacked}
%\label{plt:cOPvsKstacked}
%}
%\subfigure[I/Os vs. $k$ (CO)]{
%\hspace{-0.15in}
%\includegraphics[width=0.49\columnwidth]{c_IO_KAPA_stacked}
%\label{plt:cOPvsKstacked}
%}
%\vspace{-10pt}
%\caption{Varying number of results $k$} \centering
%\label{fig:exps_K}
%\end{figure}


\stitle{Progressiveness}. Finally, we compared the progressiveness of
\rsl and \brs algorithms. This is important for applications that
require a quick response or when the complete output is not
essential. We executed both algorithms on a workload of $|Q|$ queries
using the same default settings (refer to
Table.~\ref{tab:params}). Specifically, the x-axis represents the
percentage of reverse skyline results found so far with regards to the
total influence score. The y-axis plots the time required to report the
corresponding percentage of results, both in absolute values
(Figures~\ref{plt:aProgress},~\ref{plt:cProgress})
%,~\ref{plt:cProgress}) and as a percentage of the total time spent
(Figures~\ref{plt:aProgressPercentage},~\ref{plt:cProgressPercentage}).%,~\ref{plt:cProgressPercentage}).
The figures clearly demonstrate the superiority of \rsl algorithm in
terms of progressively reporting the query results. In particular,
\rsl requires one order of magnitude less time to output the first 5\%
of results.


\begin{figure}[t]
\centering
\subfigure[(AC)]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{a_progress}
\label{plt:aProgress}
}
\subfigure[(AC)]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{a_progress_percentage}
\label{plt:aProgressPercentage}
}
\subfigure[(UN)]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{i_progress}
\label{plt:iProgress}
}
\subfigure[(UN)]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{i_progress_percentage}
\label{plt:iProgressPercentage}
}
\subfigure[(CO)]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{c_progress}
\label{plt:cProgress}
}
\subfigure[(CO)]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{c_progress_percentage}
\label{plt:cProgressPercentage}
}
\caption{Progressiveness} \centering
\label{fig:exps_progress}
\end{figure}



\eat{
\begin{figure}[t]
\centering
\subfigure[(AC)]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{a_progress}
\label{plt:aProgress}
}
\subfigure[(AC)]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{a_progress_percentage}
\label{plt:aProgressPercentage}
}
\subfigure[(UN)]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{i_progress}
\label{plt:iProgress}
}
\subfigure[(UN)]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{i_progress_percentage}
\label{plt:iProgressPercentage}
}
%\subfigure[(CO)]{
%\hspace{-0.15in}
%\includegraphics[width=0.49\columnwidth]{c_progress}
%\label{plt:cProgress}
%}
%\subfigure[(CO)]{
%\hspace{-0.15in}
%\includegraphics[width=0.49\columnwidth]{c_progress_percentage}
%\label{plt:cProgressPercentage}
%}
\caption{Progressiveness} \centering
\label{fig:exps_progress}
\end{figure}
}

\eat{
\begin{figure*}[t]
\centering
\subfigure[(AC)]{
\includegraphics[width=0.31\textwidth]{a_progress}
\label{plt:aProgress}
}
\subfigure[(UN)]{
\includegraphics[width=0.31\textwidth]{i_progress}
\label{plt:iProgress}
}
\subfigure[(CO)]{
\includegraphics[width=0.31\textwidth]{c_progress}
\label{plt:cProgress}
}
\subfigure[(AC)]{
\includegraphics[width=0.31\textwidth]{a_progress_percentage}
\label{plt:aProgressPercentage}
}
\subfigure[(UN)]{
\includegraphics[width=0.31\textwidth]{i_progress_percentage}
\label{plt:iProgressPercentage}
}
\subfigure[(CO)]{
\hspace{-0.15in}
\includegraphics[width=0.31\textwidth]{c_progress_percentage}
\label{plt:cProgressPercentage}
}
\caption{Progressiveness} \centering
\label{fig:exps_progress}
\end{figure*}
}

\stitle{Experiments with Real Data}. Figures~\ref{plt:NBACPUvsPstacked}-\ref{plt:HOUSEIOvsCstacked} report our experimental findings on the real data sets used. The results are in accordance with our experimental study on synthetic data sets. However, notice that the differences in performance between \rsl and \brs algorithms are more intense in real data sets (especially vs. $|C|$) due to the high dimensionality. Further, there was no point to include a sensitivity analysis vs. the number of candidate products $|Q|$ for HOUSE data set, since \brs algorithm required 43 hours to run on our system for $|Q|$ = 1K. These facts further justify our motivation for a more efficient and scalable algorithm for reverse skyline queries. Overall, \rsl outperforms \brs for the single point reverse skyline query, whereas \brsl is the best choice for \kmp queries, in all experimental settings tested.

\begin{figure}[t]
\centering
\subfigure[CPU cost vs. $|P|$]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{NBA_CPU_P_stacked}
\label{plt:NBACPUvsPstacked}
}
\subfigure[I/Os vs. $|P|$]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{NBA_IO_P_stacked}
\label{plt:NBAIOvsPstacked}
}
\subfigure[CPU cost vs. $|C|$]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{NBA_CPU_C_stacked}
\label{plt:NBACPUvsCstacked}
}
\subfigure[I/Os vs. $|C|$]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{NBA_IO_C_stacked}
\label{plt:NBAIOvsCstacked}
}
\subfigure[CPU cost vs. $|Q|$]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{NBA_CPU_Q_stacked}
\label{plt:NBACPUvsQstacked}
}
\subfigure[I/Os vs. $|Q|$]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{NBA_IO_Q_stacked}
\label{plt:NBAIOvsQstacked}
}
%\subfigure[CPU cost vs. $k$]{
%\hspace{-0.15in}
%\includegraphics[width=0.49\columnwidth]{NBA_CPU_KAPA_stacked}
%\label{plt:NBACPUvsKstacked}
%}
%\subfigure[I/Os vs. $k$]{
%\hspace{-0.15in}
%\includegraphics[width=0.49\columnwidth]{NBA_IO_KAPA_stacked}
%\label{plt:NBAIOvsKstacked}
%}
\caption{Experiments - NBA Dataset} \centering
\label{fig:exps_nba}
\end{figure}


\begin{figure}[t]
\centering
\subfigure[CPU cost vs. $|P|$]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{HOUSE_CPU_P_stacked}
\label{plt:HOUSECPUvsPstacked}
}
\subfigure[I/Os vs. $|P|$]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{HOUSE_IO_P_stacked}
\label{plt:HOUSEIOvsPstacked}
}
\subfigure[CPU cost vs. $|C|$]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{HOUSE_CPU_C_stacked}
\label{plt:HOUSECPUvsCstacked}
}
\subfigure[I/Os vs. $|C|$]{
\hspace{-0.15in}
\includegraphics[width=0.49\columnwidth]{HOUSE_IO_C_stacked}
\label{plt:HOUSEIOvsCstacked}
}
%\subfigure[CPU cost vs. $|Q|$]{
%\hspace{-0.15in}
%\includegraphics[width=0.49\columnwidth]{HOUSE_CPU_Q_stacked}
%\label{plt:HOUSECPUvsQstacked}
%}
%\subfigure[I/Os vs. $|Q|$]{
%\hspace{-0.15in}
%\includegraphics[width=0.49\columnwidth]{HOUSE_IO_Q_stacked}
%\label{plt:HOUSEIOvsQstacked}
%}
\caption{Experiments - HOUSEHOLD Dataset} \centering
\label{fig:exps_house}
\end{figure}





==> greedy.tex <==
\section{A Greedy Component} 
\label{sec:greedy}

Based on the complexity of computing the subset of $k$ products, we now
seek an efficient, greedy algorithm for this problem. Our solution is
based on the generic $k$-stage Greedy Selection Algorithm (\kgcs)
provided in~\cite{HP98}, developed for finding efficient approximate
solutions to the maximum k-coverage problem.

\begin{lemma} (from~\cite{HP98})
\kgcs returns an approximate solution to the maximum
$k$-coverage problem that is guaranteed to be within a factor $1 - 1/e$
from the optimal solution.
\label{lem:kgs}
\end{lemma}

We now show how we can adapt \kgcs for the \kmp problem. The
corresponding pseudocode appears in Alg.~\ref{alg:kGCS}. \kgcs takes
as input a set of candidate products $Q$ and their associated
influence sets and returns a set $Q' \subseteq Q$, $|Q'| = k$ that
contains the candidates which formulate a $1 - \frac{1}{e}$
approximate solution to the \kmp query. \eat{Let $Opt(Q, k) =
\operatorname*{arg\,max}_{Q_k}\is(Q_k)$, with $|Q_k| = k$ and $Q_k
\subseteq Q$, i.e. $Opt(Q, k)$ represents the $k$-cardinality subset
of $Q$ that maximizes the joint influence score. Further, $Q'$
represents the solution returned by \kgcs method. Then, according to
Lemma~\ref{lem:kgs}, the following should hold:

\begin{center} $\is(Q') \geq (1 - \frac{1}{e})\is(Opt(Q, k))$ \end{center}
}
\kgcs proceeds in iterations, by adding one candidate into $Q'$
during each iteration. All candidates are examined (Lines~5-8) at
each iteration, and \kgcs selects the one that, if added in $Q'$,
results in the largest increase of the influence score of $Q'$. This
best candidate is maintained in the variable $best\_cand$ (Line~8),
and its resulting reverse skyline set is maintained in the variable
$tempRSKY$ (Line~7). \kgcs terminates after $k$ iterations and returns
$Q'$.


\begin{algorithm}[t]
\scriptsize
	\KwIn{$Q$ a set of candidates, $RSKY(q_i)$ reverse skylines of
	$q_i$, $k$}
	\KwOut{$Q'$ the most attractive set of candidates
	where $|Q'| = k$}
	\Begin
	{
	   $Q' := \varnothing; tempRSKY := \varnothing; maxRSKY := \varnothing$\;
	   \While{$|Q'| < k$}
	   {
	       $tempRSKY := maxRSKY$\;
	       \ForEach{$q_i \in Q$}
	       {
	           \If{$|RSKY(q_i) \bigcup maxRSKY| > |tempRSKY|$}
	           {
	               $tempRSKY := RSKY(q_i) \bigcup maxRSKY$\;
	               $best\_cand := \{q_i\}$\;
	           }
	       }
	       $maxRSKY := tempRSKY$\;
	       $Q := Q - best\_cand$\;
	       $Q' := Q' \bigcup best\_cand$\;
	   }
	   \Return{$Q'$}\;
	}
\caption{$k$-stage Greedy Selection Algorithm}
\label{alg:kGCS}
\end{algorithm}




\eat{
The space required to keep the influence set $RSKY(q_i), \forall q_i
\in Q$ is $O(|Q||C|)$, which may be too large to fit in memory
especially if $|C|$ is large or $d \geq 3$. To overcome this problem,
after executing \brs for each candidate, we compute an FM-sketch on
its influence set. Assuming that we use $F$ hash functions and $L$
bitmaps on each candidate, the space requirement to store all
FM-sketches is $O(F|Q|)$, that equals to $O(|Q|)$ for small values of
$F$. Then, in order to calculate the group attractiveness we exploit
the duplicate-insensitive property of FM-sketches, i.e. we only need
to apply a bitwise OR operator on the FM-sketches of each
candidate. The execution cost for \brs execution is ... and for
$\kgcs$ algorithm $O(k|Q|)$. The overall time complexity of $basic$ is
...
%
%\bga algorithm is illustrated in Fig.~\ref{fig:bga}.
}




==> introduction2.tex <==
\section{Introduction}
\label{sec:intro}

Skyline queries have been widely recognized as a practical tool in
many real world applications, such as multi-criteria decision analysis
and applications involving preference queries. Prior work mainly
focuses on helping customers select the `best\textrm{'}, based on
their preferences, product among a pool of available
products. Recently, reverse skyline queries have been
proposed~\cite{DS07}, highlighting the manufacturer's perspective,
i.e., how to determine the expected buyers of a given product. The
state of the art algorithm for answering reverse skylines queries is
the BRS algorithm, proposed in~\cite{WTW+09}.

In this work we develop novel algorithms for two important classes of
queries involving customer preferences. We first propose a novel
algorithm, termed as \rsl, for reverse skyline queries. Our \rsl
algorithm significantly reduces both the I/O cost, as well as the
computation cost, when compared to the state-of-the-art reverse
skyline algorithm \brs, while at the same time being able to quickly
report the first query results.

We then introduce a new type of queries, namely the $k$-Most
Attractive Candidates (\kmp) queries. In this type of queries, given a
set of existing product specifications $P$, a set of customer
preferences $C$ and a set of new candidate products $Q$, the \kmp
query returns the set of $k$ candidate products from $Q$ that jointly
maximizes the total number of expected buyers, measured as the
cardinality of the union of individual reverse skyline sets (i.e.,
\emph{influence sets}). Two examples of real world applications that
may benefit from answering reverse skyline and \kmp queries,
respectively, are the following:

\noindent\textbf{Market Analysis.} The marketing department of a
laptop manufacturer wants to discover which are the most
``attractive'' laptops in the market, i.e. which laptops satisfy the
preferences of the largest number of customers. Let us assume that the
manufacturer has assembled a set $P$ of all laptops available in the
market. Let us further assume that the manufacturer has conducted a
market survey and compiled a list of customers' preferences $C$ over a
laptop's attributes such as screen size, CPU, operating system etc. To
enable more effective promotion of its own products to interested
customers and adapt their advertising strategy, the marketing
department needs to discover the potential buyers for the company
products.

\noindent\textbf{Product Placement.} Consider a mobile carrier
operator that wants to introduce a set of new cell phone plans. The
operator maintains a database of existing plans, customer statistics
(i.e., voice usage duration, number of text messages, data volume
consumed per month, etc.) and a list of new phone plans under
consideration. The company is looking for the set of phone plans that
jointly would have the largest possible number of potential
subscribers.

Prior work \cite{VDKN10} has tackled a similar to \kmp problem in the
context or top-k queries. However, this approach requires learning and
precisely formulating user preference functions as weight vectors,
which is rather artificial and impractical in real life. On the other
hand, in our work each user is allowed to formulate his preferences
directly in terms of the desired product specifications. Moreover, in
contrast to our \kmp query, the total profitability of the query
result in \cite{VDKN10} is not guaranteed because multiple products
might be attractive for the same potential buyers.

Applying single point skyline approaches to solve the \kmp problem
would require calculating the reverse skyline set for each candidate,
which is prohibitively expensive for large data sets. We, thus,
propose a batched algorithms for the \kmp problem and compare its
performance against a branch-and-bound variant that we devise. Both of
these algorithms use in their core variants of our \rsl algorithm.

\noindent In brief, the contributions of this paper are:
\squishlist

\item We identify potential drawbacks, which are more evident in
high-dimensional data where the number of skyline entries is typically
larger, of the \brs algorithm. Based on our observations, we then
introduce a novel algorithm \rsl for (single) reverse skyline query
evaluation.

\item We introduce a new type of skyline query, termed as the $k$-Most
Attractive Candidates (\kmp) query; \kmp selects the set of $k$ candidate
products that jointly maximizes the total number of expected buyers.
\eat{
\item We formulate \kmp query as an optimization problem that aims to
maximize the cardinality of the union of individual influence sets.
}

\item We propose a batch algorithm for answering \kmp queries and
compare against a branch-and-bound alternative that we devise. Both of
these algorithms utilize in their core our \rsl algorithm, but
significantly improve upon naive techniques that process all candidate
products individually.  \eat{
\item We provide greedy approximation techniques for determining the
best $k$ candidates from the set of all possible $k$-cardinality
subsets.
}
\item We perform an extensive experimental study using both synthetic
and real data sets. Our study demonstrates that (\emph{i}) our \rsl algorithm
outperforms the \brs algorithm, for the reverse skyline problem, in
terms of I/O, CPU cost and progressiveness of the output, and (\emph{ii}) that our proposed batch algorithm outperforms
 naive approaches that process each candidate individually.

\squishend



This paper proceeds as follows.
Section~\ref{sec:prelim} reviews background information and
definitions, while also describing the current state-of-the-art BRS
algorithm for computing reverse skylines. Section~\ref{sec:rsl}
presents our \rsl algorithm and Section~\ref{sec:kmp} introduces the
\kmp queries. In Section~\ref{sec:kmp_algs}
%and~\ref{sec:branch_bound} we present our batch algorithms for \kmp
query evaluation, and in Section~\ref{sec:greedy} we present a greedy
method for discovering the best $k$ candidate products.
Section~\ref{sec:exps} provides our experimental
results. Section~\ref{sec:related} reviews related work, while
Section~\ref{sec:conclusion} presents concluding remarks.


==> prelim.tex <==
\section{Preliminaries}
\label{sec:prelim}

In this section we first provide some necessary definitions in
Section~\ref{sec:rskylines}. In Section~\ref{sec:inf_region} we then
present the notion of influence sets and properties regarding
influence sets, while in Section~\ref{sec:brs} we describe the state
of the art \brs algorithm for computing influence
sets. Table~\ref{tab:notation} summarizes the most frequently used
notation of this paper. The corresponding definitions are presented in
appropriate areas of the text.


%\vspace{10pt}

\subsection{Single Point Reverse Skylines}
\label{sec:rskylines}

\begin{figure*}[t]
\centering
\begin{tabular}{lcr}
\hspace{-10pt}\begin{minipage}{0.36\textwidth}
\subfigure[Dynamic Skyline of $c_1$]{
\includegraphics[width=0.45\textwidth]{exam_customer1}
\label{fig:exam_customer1}
}
\subfigure[Dynamic Skyline of $c_2$]{
\includegraphics[width=0.45\textwidth]{exam_customer2}
\label{fig:exam_customer2}
}
\subfigure[Dynamic Skyline of $c_3$]{
\includegraphics[width=0.55\textwidth]{exam_customer3}
\label{fig:exam_customer3}
}
\subfigure[Dynamic Skylines and Influence Sets]{
\includegraphics[width=0.35\textwidth]{exam_legend}
\label{fig:exam_legend}
}
\caption{Dynamic Skylines example}
\label{fig:exam_rss}
\end{minipage}
&
\begin{minipage}{0.19\textwidth}
\subfigure[Transformed space to $\Omega_0$ with respect to $q$]{
\includegraphics[width=\textwidth]{first_quadrant}
\label{fig:first_quadrant}
}
\subfigure[Midpoints with respect to $q$]{
\includegraphics[width=\textwidth]{midpoints}
\label{fig:midpoints}
}
\caption{Influence region of $q$}
\label{fig:exam_influence}
\end{minipage}
&
\begin{minipage}{0.42\textwidth}
\subfigure[Example MBB]{
\includegraphics[width=0.46\textwidth]{mbb_dom}
\label{fig:mbb_dom}
}
\subfigure[Lower bound for $\ir(q)$]{
\includegraphics[width=0.46\textwidth]{lower_frontier}
\label{fig:lower_frontier}
}
\subfigure[Upper bound for $\ir(q)$]{
\includegraphics[width=0.46\textwidth]{upper_frontier}
\label{fig:upper_frontier}
}
\subfigure[$e_c$ w.r.t $E_P$]{
\includegraphics[width=0.46\textwidth]{frontier_relations}
\label{fig:frontier_relations}
}
\caption{Influence Regions}
\label{fig:mbb_dominance_sides}
\end{minipage}

\end{tabular}
\end{figure*}


\begin{table}[t]
\begin{center}
\caption{Notation} %\centering
\label{tab:notation}
\newcommand\T{\rule{0pt}{2.6ex}}
\vspace{2pt}\scalebox{0.74}{
%\begin{scriptsize}
\begin{small}
\begin{tabular}{|l|p{3.2in}|}
\hline
\multicolumn{1}{|c|}{\textbf{Symbol}} \T& \textbf{Definition}\\ \hline\hline
$P$, $C$, $Q$ \T     & set of products, customers, candidate products \\ \hline %%
$p_i \prec_c p_j$ \T & product $p_i$ dominates $p_j$ with respect to customer $c$ \\ \hline %%
$m_i(q)$ \T          & midpoint of $p_i$ with respect to $q$ \\ \hline %%
$T_P$, $T_C$, $T^A_C$ \T      & R-tree of products, R-tree of customers, aR-tree of customers \\ \hline %%
$e_p$, $e_c$ \T      & an entry corresponding to a node of $T_P$, $T_C$ \\ \hline %%
$e_x^-(q)$, $e_x^+(q)$ \T & min-corner and max-corner of $e_x$ (w.r.t. $q$) \\ \hline %%
$SKY(c)$ \T         & skyline with respect to customer $c$ \\ \hline %%
$RSKY(q)$ \T         & influence set of candidate $q$ \\ \hline %%
$IS(q)$ \T          & influence score of candidate $q$ \\ \hline %%
$IR(q)$ \T          & influence region of candidate $q$ \\ \hline %%
$E_P(q)$, $E_C(q)$ \T & priority queue on active entries for $q$ \\ \hline %%
$L$, $U$ \T           & set of min-corners, minmax-corners for $E_P(q)$\\ \hline %%
%$RSKY^-(q)$, \T       & \multirow{2}{*}{lower and upper bound of $RSKY(q)$} \\  %%
%$RSKY^+(q)$ & \\ \hline %%
$IS^-(q)$, $IS^+(q)$ \T & lower and upper bound of $\is(q)$ \\ \hline %%
$IR^-(q)$, $IR^+(q)$ \T & lower and upper bound of $\ir(q)$ \\ \hline %%
$RSKY(Q)$ \T & joint influence set of $Q$ \\ \hline %%
$IS(Q)$ \T & joint influence score of $Q$ \\ \hline %%
\end{tabular}
%\end{scriptsize}
\end{small}
}
%\vspace{-15pt}
%\vspace{-15pt}
\end{center}
\end{table}


%Consider the following motivating example: The marketing department of a laptop manufacturer wants to discover which are the most `attractive\textrm{'} laptops in the market, i.e. which laptops satisfy the preferences of the largest number of customers. Assume that the manufacturer has assembled a set $P$ of all laptops available in the market. Further, they have conducted a market survey and compiled a list of customers' preferences $C$.

Consider two sets of points, denoted as $P$ and $C$, in the same
$D$-dimensional space. We use lower-case symbols to denote an item
that belongs to the corresponding upper-case set, e.g., $p \in P$. We
refer to each point $p \in P$ as a \emph{product}. Each product is a
multi-dimensional point, with $p_i$ denoting the product's value for
dimension (attribute) $A_i$. For example, assuming that products are
notebooks, the dimensions of $p_i$ may correspond to the notebook's
price, weight, CPU speed, screen size, etc. Further, each point $c \in
C$ represents a customer's preferred notebook specifications that he
would be interested in; we refer to each point $c$ as a
\emph{customer}.

Clearly, for some of the dimensions there exists a clear preference
(i.e., an optimal value) for all customers. In our notebook scenario,
price and weight should be as low as possible (amongst two notebooks
with all the other characteristics being identical, it is conceivable
that customers would prefer the most economic/light alternative),
whereas RAM size should be as large as possible. However, note that
there is no objectively optimal value for CPU speed and screen size. A
large screen is more practical but it also compromises
portability. Similarly, faster CPUs increase heat and fan noise and
may decrease battery life. Thus, while one customer might prefer a
notebook with 13" screen, another customer might prefer one with a
15,4" screen. In general, customers are more interested to the
products that are closer to their preferences. In order to capture the
preferences of a customer $c$ the notion of dynamic dominance among
products has been introduced.

\begin{definition}
(Dynamic Dominance) (from \cite{DS07}): Let $c \in C$, $p, p' \in
P$. A product $p$ dynamically dominates $p'$ with respect to $c$,
denoted as $p \prec_c p'$, iff for each dimension $|p_i - c_i| \leq
|p'_i - c_i|$ and there exists at least one dimension such that $|p_i
- c_i| < |p'_i - c_i|$.
\label{def:dynamic}
\end{definition}

Note that this definition can accommodate dimensions with objectively
optimal values (static dominance) where smaller (larger) values are
preferred by simply setting $c_i$ to the minimum (resp. maximum) value
of dimension $A_i$. For example, assuming that lighter notebooks are
preferred, we can simply set for all customers $c_{weight} = 0$.

\begin{definition}
(Dynamic Skyline) (from \cite{DS07}): The dynamic skyline with respect
to a customer $c \in C$, denoted as $SKY(c)$, contains all products $p
\in P$ that are not dynamically dominated with respect to $c$ by any
other $p' \in P$.
\end{definition}

Consider a set of existing products $P=\{p_1, p_2, $ $p_3, p_4\}$ and
customers $C=\{c_1, c_2, c_3\}$. Figure~\ref{fig:exam_customer1}
illustrates the dynamic skyline of $c_1$ that includes notebooks $p_2$
and $p_4$, in a sample scenario of 2-dimensional preferences that
reference the CPU speed and the screen size of a notebook. Points in
the shaded areas are dynamically dominated by points belonging to the
dynamic skyline of $c_1$. Notice that, since we are interested in the
absolute distance between products, a product might dominate other
products that belong to different quadrants with respect to a
customer. For example, $p_1$ and $p_3$ in the upper right quadrant are
dynamically dominated by $p_2$ in the lower right quadrant because
$p_2$ has a CPU speed and a screen size that are both closer to $c_1$
than the corresponding characteristics of $p_1$ and of
$p_3$. Figures~\ref{fig:exam_customer2} and \ref{fig:exam_customer3}
illustrate the dynamic skylines of customers $c_2$ and $c_3$
respectively.




\eat{
\begin{figure}[t]
\centering
\subfigure[Dynamic Skyline of $c_1$]{
\includegraphics[width=0.46\columnwidth]{exam_customer1}
\label{fig:exam_customer1}
}
\subfigure[Dynamic Skyline of $c_2$]{
\includegraphics[width=0.46\columnwidth]{exam_customer2}
\label{fig:exam_customer2}
}
\subfigure[Dynamic Skyline of $c_3$]{
\includegraphics[width=0.50\columnwidth]{exam_customer3}
\label{fig:exam_customer3}
}
\subfigure[Dynamic Skylines and Influence Sets]{
\includegraphics[width=0.32\columnwidth]{exam_legend}
\label{fig:exam_legend}
}
\caption{Dynamic Skylines example}
\label{fig:exam_rss}
\end{figure}
}

Now we highlight the product's perspective by introducing the
definition of \emph{bichromatic reverse skylines}.

\begin{definition}
(Bichromatic Reverse Skyline) (from \cite{LC08}): Let $P$ be a set of products and $C$ be
a set of customers. The bichromatic reverse skyline of $p$, denoted as
$RSKY(p)$ contains all customers $c \in C$ such that $p \in SKY(c)$.
\end{definition}

In other words, the bichromatic reverse skyline of a product $p$
contains all customers $c$ that find $p$ as `attractive\textrm{'}. In
the following we will refer to the bichromatic reverse skyline of $p$
as the \emph{influence set} of $p$. Figure~\ref{fig:exam_legend}
illustrates the influence sets of products $p_1$, $p_2$, $p_3$ and
$p_4$.

%The following lemma can be easily proved:
%
%\begin{lemma} (from \cite{DS07})
%Given a customer $c$, a candidate $q$ and a set of competitor products $P$, $c$ belongs to the influence set $RSKY(q)$ of $q$ iff $\not\exists p_i \in P$ such that $p_i$ lies inside the rectangle defined having $c$ at its center and $q$ as one corner.
%\label{lem:rsky}
%\end{lemma}
%
%To better illustrate, Fig.~\ref{fig:region} draws a set of customers $c_i$ and a rectangle that has one of the examined customers, i.e. $c_2$, at its center and $q$ as one of its corners.
%
%\begin{figure}[h!]
%\centering
%%\subfigure[Midpoint orthant skylines of $q_1$]{
%\includegraphics[width=0.48\columnwidth]{gma_props}
%\label{fig:pruning}
%%}
%\caption{Interesting Region of $c_i$}
%\label{fig:region}
%\end{figure}
%
%If $\exists p_i \in P$ that lies inside the rectangle, then it follows that $|p_{i_j} - c_{2_j}| < |q_j - c_{2_j}|$, for all dimensions $1 \leq j \leq d$. Therefore, according to Def.~\ref{def:dynamic}, $p_i \prec_{c_2} q$ and $c_2 \not\in RSKY(q)$.


Clearly, the cardinality of the influence set $RSKY(p)$ is a useful
metric of the product's impact in the market. We will refer to
$|RSKY(p)|$ as the \emph{influence score} $\is(p)$. In our example
$\is(p_1) = 2$, $\is(p_2) = 2$, $\is(p_3) = 1$ and $\is(p_4) = 1$.

%Returning to our example, the influence set of $p_1$ is $c_2, c_3$.
%
%\begin{definition}
%(Influence Score): For any product $p \in P$, its influence score $IS$ is equal to the cardinality of its influence set $RSKY(p)$, i.e. $\is(p)= |RSKY(p)|$.
%\end{definition}




\subsection{Influence Region}
\label{sec:inf_region}

Consider a new product $q$. The new product partitions the
$D$-dimensional space into $2^D$ orthants $\Omega_i$, each identified
by a number in the range $[0, 2^D-1]$. For example, in
Figure~\ref{fig:exam_influence} where $D = 2$, $q_1$ partitions the
space in 4 orthants (quadrants). Since all orthants are symmetric and
we are interested in the absolute distance between products, we can
map all products to $\Omega_0$ as illustrated in
Figure~\ref{fig:first_quadrant}. For simplicity, we hereafter
concentrate on $\Omega_0$ with respect to a query point $q$.

\eat{
\begin{figure}[t]
\centering
\subfigure[Transformed space to $\Omega_0$ with respect to $q$]{
\includegraphics[width=0.46\columnwidth]{first_quadrant}
\label{fig:first_quadrant}
}
\subfigure[Midpoints with respect to $q$]{
\includegraphics[width=0.46\columnwidth]{midpoints}
\label{fig:midpoints}
}
\caption{Influence region of $q$}
\label{fig:exam_influence}
\end{figure}
}

For every dynamic skyline point $p_i$, let $m_i(q)$ be the midpoint of the segment connecting a query point $q$ with $p_i$. In Figure~\ref{fig:midpoints} black points $m_1$, $m_2$ and $m_4$ represent the midpoints of $p_1$, $p_2$ and $p_4$ with respect to $q$.

In the rest of this work, in order to get rid of the complication of maintaining both points and midpoint skylines, whenever we refer to a product $p_i$ we will imply the corresponding $m_i(q)$ in respect to $q$. Further, we will assume that each dynamic skyline point $p_i$ with respect to $q$ is mapped to its midpoint skyline $m_i$ on the fly.

The \emph{influence region} of a query point $q$, denoted as $\ir(q)$, is the union of all areas not dynamically dominated (\emph{anti-dominance areas}) with respect to $q$ by the midpoint skylines of $q$. The area in $\Omega_0$ that is not shaded in Figure~\ref{fig:midpoints} draws the influence region for $q$.

%Note that the midpoints themselves belong to the \ir, since a tuple cannot dominate itself.

%The following lemma comes from \cite{LC08}.

\begin{lemma} (from \cite{LC08})
A customer $c$ belongs to the influence set $RSKY(q)$ of $q$ iff $c$ lies inside the influence region of $q$ i.e., $c \in \ir(q) \Leftrightarrow c \in RSKY(q)$.
\label{lem:ir_rss}
\end{lemma}

Returning to the example of Figure~\ref{fig:midpoints}, notice that only $c_2$ lies inside $\ir(q)$. Therefore, $RSKY(q) = \{c_2\}$.

%, as also discussed in the context of Figure~\ref{fig:exam_rss}.


In our discussion hereafter, we assume that all points (either products or customer preferences) are indexed using a multidimensional index (e.g. R-trees, kd-trees etc.). Although any multidimensional index can be used instead, R-trees represent an attractive choice because of their popularity in commercial database systems. Figure~\ref{fig:mbb_dom} shows an example minimum bounding box (MBB) $e$.

%Each minimum bounding box (MBB) of the R-tree may contain an arbitrary number of points whose exact attribute values are unknown. %

\eat{
\begin{figure}[t]
\centering
\subfigure[Example MBB]{
\includegraphics[width=0.46\columnwidth]{mbb_dom}
\label{fig:mbb_dom}
}
\subfigure[Lower bound for $\ir(q)$]{
\includegraphics[width=0.46\columnwidth]{lower_frontier}
\label{fig:lower_frontier}
}
\subfigure[Upper bound for $\ir(q)$]{
\includegraphics[width=0.46\columnwidth]{upper_frontier}
\label{fig:upper_frontier}
}
\subfigure[$e_c$ w.r.t $E_P$]{
\includegraphics[width=0.46\columnwidth]{frontier_relations}
\label{fig:frontier_relations}
}
\hspace{20pt}
%\subfigure[Certain dominance relationships of all faces]{
%\hspace{-10pt}
%\includegraphics[width=0.4\columnwidth]{mbb_dom_sides}
%\label{fig:mbb_dom_sides}
%}
\caption{Influence Regions}
\label{fig:mbb_dominance_sides}
\end{figure}
}

Inside each MBB $e$, let \emph{min-corner} $e^-(c)$ denote that point
(in $e$) at the minimum distance from a query point
$q$\footnote{\scriptsize{Note that the notation does not use
$q$}}. The min-corner dominates the largest possible part of the
orthant. Further, due to the construction of an MBB, i.e., it is the
smallest possible box that encloses a set of points, an MBB has the
property that each face (i.e., side) must contain at least one point
(otherwise the box would be shrunk). The points that reside in each of
the $d$ faces closest to $q$ and are the farthest from the origin $q$
are denoted as \emph{minmax-corners}. Each MBB contains $D$
minmax-corners. Independently of how products within $e$ are
distributed, any point in $e$ certainly dominates the area that the
minmax-corners do, while at best it dominates the area that the
min-corner does.

Given a set of MBBs, we can derive two sets: the set of all min-corners denoted as $L$ and the set of all minmax-corners denoted as $U$ with respect to $q$. Figure~\ref{fig:lower_frontier} presents an example, assuming $E_P=\{{e_p}_1, {e_p}_2, {e_p}_3, {e_p}_4\}$, where $e_{p_i}$ denotes a product entry. In Figures~\ref{fig:lower_frontier},~\ref{fig:upper_frontier} black and hollow circles represent the min-corners and minmax-corners respectively and rectangles represent midpoints.

Consider the example of Figure~\ref{fig:lower_frontier}. The grey area represents a lower bound of the actual influence region $\ir^-$ and it is defined as the space not dominated by any min-corner $l \in L$. Continuing the example, in Figure~\ref{fig:upper_frontier} the grey area represents an upper bound of the actual influence region $\ir^+$, defined as the space not dominated by any minmax-corner $u \in U$. It follows \cite{WTW+09}:

\begin{lemma}
If an entry $e_c$ is dominated by any $u \in U$, i.e. $e_c$ is completely outside $\ir^+(q)$, $e_c$ certainly cannot contain any customer belonging to $\ir(q)$. Consequently, according to Lemma~\ref{lem:ir_rss}, $e_c$ does not contribute any reverse skyline point, hence it can be pruned.
\label{lem:prop1}
\end{lemma}

For example, ${e_c}_1$ in Figure~\ref{fig:frontier_relations} can be pruned because it is completely outside $\ir^+(q)$.






%The following pruning rules apply \cite{WTW+09}:
%
%\begin{enumerate}
%
%\item If an entry $e_p \in E_P$ is dominated by any $u \in SKY(U)$, $e_p$ can be removed from $E_P$, as it cannot contribute to further refining the influence region of $q$.
%
%    For example, ${e_p}_4$ in Figure~\ref{fig:lower_frontier} can be pruned because it is dominated by at least one minmax-point $u \in SKY(U)$.
%
%\item If an entry $e_c \in E_C$ is dominated by any $u \in SKY(U)$, i.e. $e_c$ is completely outside $\ir^+(q)$, $e_c$ can be removed from $E_C$ because it certainly cannot contribute any customer inside $\ir(q)$ according to Lemma~\ref{lem:ir_rss}.
%
%    For example, ${e_c}_1$ in Figure~\ref{fig:frontier_relations} is completely outside $\ir^+(q)$, hence it can be pruned.
%
%\item If there is no $e_c \in E_C$ that intersects the exclusive dominance area of an entry $e_p \in E_P$, $e_p$ can be removed from $E_P$, because expanding $e_p$ will not contribute any customers to the $RSKY(q)$.
%
%\end{enumerate}
%
%
%To better justify the last pruning rule consider $e_{p_3}$ in Figure~\ref{fig:prune_rule_a}. Observe that $e_{c_1}$ intersects the dominance area of both $e_{p_3}$ and $e_{p_2}$. Therefore, there is no need in keeping $e_{p_3}$ in $E_P$. However, in Figure~\ref{fig:prune_rule_b}, $e_{c_1}$ intersects the exclusive dominance area of $e_{p_3}$, hence $e_{p_3}$ must be expanded to refine $\ir(q)$.
%
%\begin{figure}[ht!]
%\centering
%\subfigure[$e_{p_3}$ can be removed]{
%\hspace{-13pt}
%\includegraphics[width=0.46\columnwidth]{prune_rule_a}
%\label{fig:prune_rule_a}
%}
%\subfigure[$e_{p_3}$ must be expanded]{
%\hspace{-10pt}
%\includegraphics[width=0.46\columnwidth]{prune_rule_b}
%\label{fig:prune_rule_b}
%}
%\hspace{-13pt}
%\caption{Pruning rule 3}
%\label{fig:pruning_rules}
%\end{figure}


%Now, we define as the \emph{optimistic dominance area} the union of all areas that are orthant-dominated in respect to $q$ by any of the min-corners $l \in L$ and as \emph{pessimistic dominance area} the union of all areas that are orthant-dominated in respect to $q$ by any of the minmax-corners $u \in U$. The optimistic dominance area always covers the pessimistic one.

%Therefore, we can safely assume that at least one point lies in each of the $2d$ faces of an MBB.



\subsection{The \brs Algorithm}
\label{sec:brs}


In the following we detail the state-of-the-art \emph{Bichromatic Reverse Skyline} (\brs) algorithm \cite{WTW+09} that efficiently calculates the influence set of a single query point $q$. \brs aims at minimizing the I/O cost (\emph{i}) by progressively refining the influence region of $q$ until the influence set of $q$ has been retrieved, (\emph{ii}) by applying Lemma~\ref{lem:prop1} to prune $e_c$ entries that do not contribute to $RSKY(q)$.

\brs uses two indexes, an R-tree $T_P$ on the set of products $P$ and another $T_C$ on the set of customers $C$. Initially, the algorithm inserts all root entries of $T_P$ (resp. $T_C$) in a priority queue $E_P$ (resp. $E_C$) sorted with the minimum Euclidean distance (\emph{mindist}) of each entry from $q$. \brs extracts a set $L$ of all min-corners and a set $U$ of all minmax-corners of $e_p \in E_P$. Further, in order to reduce the number of subsequent dominance checks, \brs calculates the skylines of $L$ and $U$, denoted as $SKY(L)$ and $SKY(U)$ respectively. %\footnote{Essentially, keeping only the skyline points of each set is sufficient}

%An $E_P$ entry, such as ${e_p}_4$, that is dominated by $S_P^+$, is purged. The area covered by $\ir^+$ but not $\ir^-$ is called the \ir \emph{frontier} (shown gray in Figure~\ref{fig:frontier_relations}) and denoted as $\dir = \ir^+ - \ir^-$.

In each iteration \brs expands the entry in $E_P$ with the minimum mindist from $q$ and updates the current $L$ and $U$ and their skylines $SKY(L)$ and $SKY(U)$. Then, all $e_c \in E_C$ are checked for dominance with $SKY(L)$ and $SKY(U)$. If $e_c$ is not dominated by $SKY(L)$ (i.e. it intersects $\ir^-(q)$), \brs expands $e_c$ as it will certainly contain at least one customer belonging to $\ir(q)$. Returning to Figure~\ref{fig:frontier_relations}, ${e_c}_3$ intersects $\ir^-(q)$, meaning that it contains at least one customer inside $\ir(q)$, therefore it is expanded. In contrast, if $e_c$ (such as ${e_c}_1$ in Figure~\ref{fig:frontier_relations}) is dominated by $SKY(U)$, then $e_c$ can be safely pruned according to Lemma~\ref{lem:prop1}.



Additionally, in each iteration \brs checks all $e_p \in E_P$ with the current $SKY(U)$. If an entry $e_p$ is dominated by any $u \in SKY(U)$, then $e_p$ can be removed from $E_P$, as it cannot contribute to further refining $\ir(q)$. For example, ${e_p}_4$ in Figure~\ref{fig:upper_frontier} can be pruned because it is dominated by at least one minmax-corner $u \in SKY(U)$. \brs terminates when $E_C$ becomes empty, i.e. the position of all customers either inside or outside $\ir(q)$ has been determined.


 %Further, ${e_c}_2$ lies completely inside $\ir^-(q)$, which implies that all customers in ${e_c}_2$ definitely belong to $\ir(q)$. ${e_c}_4$ in Figure~\ref{fig:frontier_relations} intersects only $\ir^+(q)$, i.e. customers within ${e_c}_4$ may or may not belong to $\ir(q)$. However, ${e_c}_4$ might be pruned in a subsequent iteration of \brs due to Pruning Rule 2, therefore it is kept in $E_C$ (and it is not expanded).




%progressively reports $IS(q)$


%Section~\ref{sec:dominance} discusses uncertain dominance,


==> problemdefinition.tex <==
\section{Problem Formulation: k-MAC Queries}
\label{sec:kmp}

After presenting our \rsl algorithm for efficiently calculating the
reverse skyline set for a single candidate, in this section we
introduce the notion of $k$-Most Attractive Candidates (\kmp)
queries. We first present a motivating sample scenario, which
highlights the importance of \kmp queries. We then formally define our
\kmp problem.

\stitle{Motivating Scenario.}  A laptop manufacturer wants to produce
$k$ new notebooks, among a set of feasible candidate laptop
configurations $Q$ proposed by the engineering department. In this
process, the manufacturer needs to consider three sets: (1) the
existing competitor products $P$, (2) the set of customers' preferred
specifications $C$, and (3) a set of candidate products $Q$. We will
refer to each $q \in Q$ as a \emph{candidate}.

Clearly, the goal of the manufacturer is to identify the
specifications that are expected to \emph{jointly} attract the largest
number of potential buyers. Please note that this is different than
simply selecting the $k$ products that are the most attractive
individually, since it does not make much sense to select products
that seem attractive to the same subset of customers.


\stitle{Problem Definition.}  \eat{{\bf Antonis: AYTO POU PARAKATW TO
8ELOUME? LEW NA TO BGALOUME: For ease of presentation, we consider, in our discussion
hereafter, each candidate $q \in Q$ separately from other
candidates. Hence, the definition of dynamic dominance and all
subsequent definitions should be modified in order to examine $P
\bigcup \{q\}$ instead of $P$, i.e. a point $p \in P \bigcup \{q\}$
belongs to $SKY(c)$ iff $\not\exists p' \in P \bigcup \{q\}$ such that
$p' \prec_c p$.
%We raise this assumption in Section~\ref{sec:group_kma} where the influence sets of two (or mode) candidates overlap.
}
}
We first define the \emph{joint influence set} for a set of candidates
$Q$. We then define the notion of the \emph{joint influence score} and
introduce the \emph{$k$-Most Attractive Candidates (\kmp)
query}.


\begin{definition}
(Joint Influence Set): Given a set of products $P$, a set of customers
$C$ and a set of candidates $Q$, the joint influence set of $Q$,
denoted as $RSKY(Q)$, is defined as the union of individual influence
sets of any $q_i \in Q$.

\vspace{3pt}

\begin{center}\begin{small} $RSKY(Q) = \displaystyle \bigcup_{q_i \in Q} RSKY(q_i)$ \end{small}\end{center}
\end{definition}

\vspace{3pt}

Following the above definition, the \emph{joint influence score}
$\is(Q)$ for a set of candidates $Q$ is equal to the size
($|RSKY(Q)|$) of the joint influence set of $Q$.

We now introduce the \emph{$k$-Most Attractive Candidates} (\kmp)
query as follows:
\begin{definition}
$k$-Most Attractive Candidates (\kmp) query): Given a set of products $P$, a set
of customers $C$, a set of candidates $Q$ and a positive integer $k >
1$, determine the subset $Q_i \subseteq Q$, such that $|Q_i| = k$ and
the joint influence score $\is(Q_i)$ of $Q_i$ is
maximized.\footnote{Note that since the joint influence score of a set
of candidates is non-decreasing when adding new members in the set,
the optimal solution in this problem is guaranteed to contain exactly
$k$ candidates.}
\end{definition}

Obviously, the $\gkmp{1}$ problem returns the most attractive
candidate. Returning to Figure~\ref{fig:exam_rss}, assuming that the
four products represent the four candidates, the solution to a
$\gkmp{2}$ query could return as solution either the set $\{p_1,
p_2\}$, or the set $\{p_1, p_4\}$ or $\{p_2, p_3\}$, all of them
having a joint influence score of 3. In case of ties, these ties can
be resolved arbitrarily.  \eat{In case of ties, we will assume that
the set with the maximum $\displaystyle \sum_{q_i \in Q} |RSKY(q_i)|$
is selected, i.e. $\{p_1, p_2\}$. }

Unfortunately, answering \kmp queries is non-trivial. This problem can
trivially be reduced to the more general \emph{maximum k-coverage}
problem. Thus, even if we consider the much simpler problem where all
the influence sets of all candidates have been computed, an exhaustive
search over all potential $k$ cardinality subsets of $Q$ is NP-hard.




==> related.tex <==
\section{Related Work}
\label{sec:related}


The skyline query returns the set of not dominated objects,
corresponding to the Pareto optimal set. \cite{BKS01} introduce
skyline queries in the context of database research, also presenting
various external memory algorithms. %The most well-known method is Block Nested Loops (BNL), which checks each point for dominance against the entire dataset.
%Furthermore, the authors describe an index-based approach, as well as an extension of the main memory multidimensional divide and conquer algorithm of \cite{PS85}.
Since then, several non-indexed \cite{CGGL03, GSG07, BCP08} and
indexed-based algorithms \cite{KRR02, PTFS05, LZLL07} have been
presented in skyline research literature.

Assuming a set of products $P$, the dynamic skyline \cite{PTFS05}
contains all products $p \in P$ that are `attractive\textrm{'}
according to a customer's preferences. In order to capture the
manufacturer's perspective, \cite{DS07} introduces reverse skyline
query, which returns all customers $c \in C$ that would find a product
$p$ as `attractive\textrm{'}, and proposes a branch and bound
extension of the BBS algorithm \cite{PTFS05} that reduces the search
space. \cite{LC08} improves upon \cite{DS07} by providing tighter pruning
rules based on midpoint skylines (Section~\ref{sec:inf_region}) and
proposes algorithms for calculating reverse skylines on uncertain
data. \cite{WTW+09} introduces the \brs algorithm (Section~\ref{sec:brs})
which exploits some additional optimizations that are possible for the
case of certain data.

Several other skyline-based approaches that focus on the
manufacturer's view have been proposed as well. DADA \cite{LOTW06}
aims to help manufacturers position their products in the market,
based on dominance relationship analysis. A product $p$ satisfies a
customer $c$ iff $p$ dominates $c$. %Three query types are proposed; for instance, given a plane $L$ the \emph{Linear Optimization Query (LOQ)} returns the point $p \in L$ that satisfies (i.e. dominates) the largest number of customers.
However, DADA does consider user preferences, hence it can only be used on static dimensions,
i.e. those having optimal values that are independent of user preferences.
Another approach similar in motivation to our work is
\cite{WWI+09} that addresses the problem of identifying competitive
packages formulated by combining individual products, such as a flight
and a hotel. A package is competitive if it is not dominated by any
other package. In \cite{WWP11} the authors extend this work by
proposing methods to calculate the $k$ most profitable products,
i.e. those that maximize the profit gain measured as the package
price. Apart from the different application setting from our work, \cite{WWI+09, WWP11} do not consider dynamic
dimensions or multiple customers either. In contrast, our work
captures the profitability of each product in terms of the
number of potential buyers.

Assuming that user preferences are formulated as functions, the skyline set will
always include the top-1 result for any preference function that is monotone.
Due to the difficulty to come up with a precise preference function in many scenarios,
skyline queries have been particularly useful in preference queries.
Due to the difficulty to come up with a precise preference function in many scenarios,
skyline queries have been particularly useful in preference queries.
%Other skyline points capture the importance of different dimensions for different users, for example a preference for cheaper product of user $A$ vs. a
%preference for a faster CPU of user $B$.
On the other hand, assuming that a linear preference function
is available, \emph{top-k queries} \cite{CG99, FLN01} provide
an alternative solution to skylines.
%The output of a top-k query returns the $k$ products with the highest score according to a user's
%preference function, i.e. those that best satisfy the user's preferences.

Given a product $p$ and set of user preference functions
$W$ formulated as weight vectors, \cite{VDKN10} introduces
\emph{reverse top-k queries}. In analogy to reverse skylines, the
reverse top-k query returns those weight vectors such that $p$ belongs
to their top-k query results. \cite{VDNK10} extends \cite{VDKN10} by
addressing the problem of discovering the top-m products that
maximize the cardinality of their reverse top-k set. Although the
spirit of \cite{VDKN10} is similar to our approach, it
requires learning and precisely formulating user preference functions
as weight vectors, which is rather impractical in real life. On the
other hand, in our work each user is allowed to formulate her preferences
directly in terms of the desired product specifications. Moreover, in contrast
to our \kmp query, the total profitability of the query result in \cite{VDKN10}
is not guaranteed because multiple products might be attractive for
the same potential buyers.


Finally, the skyline query exhibits some similarities with the
\emph{nearest neighbor query} ($\nn$) \cite{RKV95}. %proposed in
spatial databases.  Given a set of spatial objects (e.g. facilities)
$P$ and a query point $q$ (e.g. a user's spatial location), the
\emph{$k$-nearest neighbor query} ($k\nn(q)$) contains the $k$ objects
$p \in P$ having the minimum spatial distance to $q$. Further, given
an object $p$ and a set of customers $C$, the \emph{bichromatic
reverse nearest neighbor query} ($\rnn(p)$) \cite{KM00} returns the
customers $c \in C$ whose \nn contains $p$. The work in \cite{XZKD05}
selects the $k$ objects from a set $P$ inside a given spatial region
$Q$, such that they have the largest \rnn set. Finally, a more recent
work \cite{WOY+09} addresses the problem of identifying the region to
establish a new facility so that the size of its \rnn set is
maximized. %The authors construct a set of candidate sites, termed
\emph{vantage points}, so that the most influential among them define
the optimal region.  The problem formulation and the proposed
solutions are similar to our approach. However none of these methods
can be directly applied to our setting, because the
`attractiveness\textrm{'} of each product $p$ is based on its
dominance relationships with other competitor products with respect to
a customer $c$, rather than its distance from $c$.

\stitle{Acknowledgements}. This research has been co-financed by the European Union (European Social Fund - ESF) and Greek national funds through the Operational Program "Education and Lifelong Learning" of the National Strategic Reference Framework (NSRF) - Research Funding Program: Heracleitus II. Investing in knowledge society through the European Social Fund.




%Maximum coverage problem ... \cite{LYZZ07, TDLP09}

%\cite{MDHM08} propose an algorithm that selects the subset of attributes that maximizes the 'visibility' of a new product in the market. In \cite{WXMH09}, promotion analysis for business intelligence is studied, which discovers for a given point the subspaces in which it is highly ranked. A related problem is that of finding the top-k most interesting regions for promotion of an object \cite{WSLH10}.

%Analogies with RNN queries ... \cite{RKV95, KM00, SRAA01, TPL04, XZKD05}

%Given a query object q, reverse nearest neighbor queries [4] aim to retrieve those objects that have q as their nearest neighbor based on a similarity function. These objects are said to be influenced by q. Finding the region in space that maximizes the size of bichromatic reverse nearest neighbor is studied in [11]. The notion of influence has also been used by other approaches, in order to identify the best objects in a dataset. In spatial databases, an interesting problem is to compute the top-t most influential spatial sites [14], where the influence of an object is defined as the total weight of its reverse nearest neighbors. We argue that in the context of studying the impact of products in the market, our definition of influence is meaningful and intuitive, since it inherently integrates the most important factor for assessing the impact, namely the visibility of the product based on user preferences (in terms of top-k queries).

%There are apparent analogies between nearest neighbor (NN) queries \cite{RKV95} (and their variations) in spatial databases, and skylines; Table~\ref{tab:analogies} summarizes the concepts. Given a set of sites $S$, the \emph{nearest neighbor set} $\nn(c)$ of some client $c$ contains the sites $s \in S$ which are closest to $c$ (there may exist multiple clients at the same minimum distance to $s$), i.e., the sites that are \emph{spatially interesting} for $c$. Given $S$ and a set of clients $C$, the \emph{reverse nearest neighbor set} \cite{KM00} $\rnn(s)$ of a site $s \in S$
%contains the clients $c \in C$ whose NN set contains $s$, i.e., the points that are \emph{spatially interested} in $s$. The Voronoi cell of a site $s$ is the locus of points that are closer to $s$ than any other site. Therefore, all clients inside the cell of $s$ belong to its $\rnn(s)$. Note that in contrast to dominance-based influence regions (see Section~\ref{sec:inf_region}), Voronoi cells do not overlap. Therefore, a client (unless it lies on the border of a cell) is associated with a single site. On the other hand, a product can be in the skyline of many buyers. \cite{SRAA01} proposes a method to compute $\rnn(s)$ based on an approximation of $s$' Voronoi cell. For the \emph{monochromatic} case, where clients also act as sites, \cite{TPL04} traverses an R-tree built on $S$ to progressively construct the Voronoi cell of $s$, while pruning entries that cannot be in the $\rnn(s)$. The work in \cite{XZKD05} selects the $k$ sites among a set $S$ inside a given spatial region $Q$ that have the largest RNN set. The problem formulation and the proposed solution is similar to \emph{k-MA} queries. The authors use aggregate R-trees on the sets of sites and clients and insert their entries into heaps. In addition, they establish lower and upper bounds for the influence count of sites and propose an expansion strategy based on the estimated importance of heap entries.

%A more recent work \cite{WOY+09} addresses the continuous version of the above problem, in which the goal is to identify the region to establish a new site so that its \rnn is maximized. The authors construct a set of candidate sites, termed \emph{vantage points}, so that the most influential among them can uniquely identify the optimal region.

%\begin{table}[h!]
%\centering%%
%\caption{NN -- skyline analogies}
%\begin{scriptsize}
%\begin{tabular}[b]{|l|l|}
%%\begin{tabular}[b]{ll}
%\hline
%\textbf{NN}& \textbf{Skyline}\\ \hline\hline
%Site, Client & Product, Customer\\ \hline
%Distance & Dominance\\ \hline
%Nearest neighbor of a client \cite{RKV95} & Skyline of a customer \cite{BKS01}\\ \hline
%Reverse NN of a site \cite{KM00} & Reverse skyline of a product \cite{DS07}\\ \hline
%Voronoi cell of a site \cite{SRAA01} & Influence region of a product\\ \hline
%Most influential sites \cite{XZKD05} & Most attractive products\\ \hline
%\end{tabular}
%\end{scriptsize}
%\label{tab:analogies}
%\end{table}







%The skyline computation, or finding the maxima in a set of vectors, has a long history in the area of computational geometry \cite{KLP75,PS85}. The skyline points correspond to the Pareto accumulation or composition of all attribute preferences, as defined in \cite{K02,C03}. The work of \cite{BKS01} introduces secondary memory algorithms, including a block nested loops (BNL) approach. The SFS algorithm \cite{CGGL03} and its extensions (i.e., LESS \cite{GSG07} and SaLSa \cite{BCP08}) improve on BNL by presorting points according to a monotone preference function. Index-based approaches, such as BBS \cite{PTFS05} that uses an R-tree or \cite{LZLL07} that builds a B-tree based on the z-order of tuples, prune multiple points without having to visit them.


%Many skyline-based variations have been recently studied. The notion of probabilistic skylines \cite{PJLY07} applies to the case of uncertainty in data. The \emph{multi-source skyline query} \cite{DZS07,SS06} retrieves the records not dominated with respect to a set of exemplar tuples. For the case of categorical, or nominal attributes, where preferences define only partial (instead of total) orders, several approaches have been proposed \cite{CET05, SDKT08, WFP+08, SPP09}. Methods for computing the skyline over distributed data are presented in \cite{BGZ04, VDKV07, CLX+08}. To address the problem of large skylines in high dimensional and anti-correlated datasets, the works in \cite{CJT+06,LYZZ07,TDLP09} return a bounded set of points that best capture dominance relationships.

%A similar in spirit work to ours but applied to a different problem setting is \cite{WWI+09}. The authors wish to identify competitive packages constructed by bundling individual products, e.g., a flight and a hotel. A package is called competitive if it is not dominated by other similarly constructed or existing packages. The main challenge is to identify the competitive packages without generating all possible combinations. Note that the method in \cite{WWI+09} does not consider multiple buyers and hence cannot measure the importance of a package in terms of the expected demand (in terms of the number of interested buyers).

%Given a query object q, reverse nearest neighbor queries [4] aim to retrieve those objects that have q as their nearest neighbor based on a similarity function. These objects are said to be influenced by q. Finding the region in space that maximizes the size of bichromatic reverse nearest neighbor is studied in [11]. The notion of influence has also been used by other approaches, in order to identify the best objects in a dataset. In spatial databases, an interesting problem is to compute the top-t most influential spatial sites [14], where the influence of an object is defined as the total weight of its reverse nearest neighbors. We argue that in the context of studying the impact of products in the market, our definition of influence is meaningful and intuitive, since it inherently integrates the most important factor for assessing the impact, namely the visibility of the product based on user preferences (in terms of top-k queries).


%[cite spatial join, capacity based spatial assignment?]




==> rsl.tex <==
\section{The \rsl Algorithm}
\label{sec:rsl}

In this section, we detail the drawbacks of \brs and then propose our
more efficient reverse skyline algorithm, \rsl.

\begin{figure}[t]
\centering
\includegraphics[width=0.35\columnwidth]{redundant_IO}
\caption{Expanding $e_{p_2}$ entry in \brs is redundant, as it cannot
refine $e_{c_1}$}
\label{fig:redundant_IO}
\end{figure}


\subsection{\brs Shortcomings}
\label{sec:shortcomings}

\stitle{Complexity Analysis}. Let $p_k$, $c_k$ denote the sizes of
active lists $E_P$ and $E_C$, respectively, after the $k$-th iteration
of the \brs algorithm. The worst-case cardinality of $p_k$ and $c_k$
are $|P|$ and $|C|$ respectively. In each iteration, the \brs
algorithm maintains both $SKY(L)$ and $SKY(U)$, two sets with $O(|P|)$
and $O(D|P|)$ entries respectively, where $D$ is the dimensionality of
the data set.  \brs then checks for dominance each entry in $E_P$ and
$E_C$ with $SKY(L)$ and $SKY(U)$. Thus, each iteration entails
$O(D^2|P| \times (|P| + |C|))$ comparisons\footnote{Recall that each
dominance check requires $D$ comparisons}. \eat{Overall, assuming $m$
iterations, the time complexity of \brs algorithm is $O(md|P|(|P| +
|C|))$.}

Clearly, the processing cost of \brs depends heavily on the size of
the intermediate $SKY(L)$ and $SKY(U)$ sets. Godfrey~\cite{G04} shows
that for a uniformly distributed data set, the size of the skyline set
is $\Theta(\frac{(lnN)^{D-1}}{(D-1)!})$, where $N$ is the data set
cardinality.  Thus, for higher dimensional data, or in larger data
sets, the processing cost of maintaining the lower and upper bounded
skylines\eat{ (especially for several iterations)} becomes
prohibitively expensive. As we also demonstrate in our experiments,
\brs becomes impractical when $N \geq 10^6$ or $D \geq 4$. Motivated by
the above analysis, we seek to develop in this section a more
efficient and scalable reverse skyline algorithm, which will eliminate
the dependency on the $SKY(L)$ and $SKY(U)$ sets, thus being able to
handle high dimensional data, or, in general, data where the size of
(reverse) skylines is large.  \eat{In contrast, we propose a novel
reverse skyline algorithm that is more efficient in terms of
processing time and scales better as the number of dimensions or data
cardinality increase.}

\stitle{Visiting Order}. \brs algorithm performs a synchronous
traversal on the $T_P$ and $T_C$ indexes, which are built on product
and customer points, respectively. The execution of the \brs algorithm
follows a monotonic order based on the Euclidean distance of $e_p$
entries from $q$. This visiting order ensures that the number of I/O
operations on $T_P$ is minimized. However, it cannot guarantee that
the total number of I/Os (both on $T_P$ and $T_C$) is optimal.


We argue that, depending on the relative position of $e_p$ and $e_c$
with respect to $q$, a different visiting order might entail fewer
I/Os than those required by the \brs
algorithm. Fig.~\ref{fig:redundant_IO} illustrates one such scenario,
where the nodes $e_{p_2}$ and $e_{c_1}$ have not been expanded yet. In
this scenario, \brs would proceed by expanding $e_{p_2}$, thus
revealing the entries $e_{p_4}$ and $e_{p_5}$. Unfortunately,
$e_{c_1}$ is not affected by this refinement and it still has to be
accessed. However, if we first expand $e_{c_1}$, this operation would
reveal $e_{c_2}$ and $e_{c_3}$, which can be pruned by $p_1$ and $p_3$
respectively, eliminating the need to access $e_{p_2}$. Clearly, in
this scenario the I/O operation on $e_{p_2}$ was redundant.\eat{ \brs
would perform 2 I/Os, whereas only one (i.e on the customer entry) was
necessary.} In this work, we introduce a new reverse skyline algorithm
that follows a visiting order based on a customer entry's tree level
(primary sort criterion) and Euclidean distance (secondary sort
criterion) from $q$. Following the proposed visiting order, a product
entry will be accessed only as long as it is necessary in order to
determine if a customer point belongs to $RSKY(q)$, which leads to
fewer total I/O operations on both indexes.


\stitle{Progressiveness}. \brs algorithm iteratively refines
$\ir^-(q)$ and reports the customer points that lie inside
$\ir(q)$. In order to retrieve the first result, several iterations of
\brs might be required, which is a not desirable property for
applications that require a quick response that contains only a
fraction of the total output. We thus seek to develop an algorithm
that reports the first results faster than \brs algorithm and which is
more progressive in terms of the fraction of output reported.


\subsection{\rsl Algorithm}
\label{sec:rsl_alg}

We now propose our \rsl (Reverse Skyline Algorithm), which aims to
eliminate the shortcomings outlined above. In particular, our \rsl
algorithm:

\begin{itemize}
\item Does not require the maintenance of the $SKY(L)$ and $SKY(U)$
sets, and is, therefore, significantly less expensive in terms of
processing cost.
\item It checks one customer entry per iteration following a visiting
order based on the entry's tree level (primary sort criterion) and
Euclidean distance (secondary sort criterion) from $q$.
\item It accesses a $e_p$ entry only if it is necessary in order to
determine if a customer point belongs to $RSKY(q)$.
\end{itemize}

\stitle{Data Structures Used and Basic Intuition.}
\rsl maintains five data structures for its operation:
\begin{itemize}
\item A priority queue $E_P$ on the set of active products entries
\item A priority queue $E_C$ on the set of active customer entries
\item A R-tree $T_P$ on the set of products $P$
\item A R-tree $T_C$ on the set of customers $C$
\item A set $SKY(q)$ of the currently found midpoint skylines
\end{itemize}
The two priority queues are sorted based on a dual sorting criterion:
primarily, based on the tree level of the stored entries and,
subsequently, using the mindist of each entry from $q$. Thus, leaf
entries are given higher priority and are processed first, while the
examination of non-leaf entries is postponed as much as possible. By
first processing all leaf $e_c$ entries, the algorithm may reveal a
midpoint skyline, which will be subsequently used to prune a non-leaf
$e_c$, thus avoiding an access on $T_C$. The same intuition holds for
$e_p$ entries as well; when a $e_c$ entry is checked for dominance
with $E_P$, first all leaf $e_p$ entries will be examined. As long as
no non-leaf $e_p$ dominates $e_c$, only then will \rsl proceed to
expand the nearest non-leaf $e_p$ entry to $q$. This change in the
visiting order of $E_P$ reduces the number of accesses on $T_P$ as
well.


\eat{First we outline the basic idea behind \rsl algorithm. \rsl aims
to avoid expanding $e_p$ unless it is necessary for deciding the
inclusion of a $e_c$ entry in $\is(q)$. Further, \rsl maintains two
priority queues $E_P$ on the set of products $P$ and another $E_C$ on
the set of customers $C$. Both priority queues are sorted first based
on the tree level of $e_x$\footnote{\scriptsize{$e_x$ stands for
either $e_p$ or $e_c$}}, and then using the mindist of $e_x$ from
$q$. The intuition is to postpone the examination of non-leaf $e_c$
entries. First all leaf $e_c$ are examined. This examination might
reveal a midpoint skyline that will be subsequently used to prune a
non-leaf $e_c$, hence avoiding an access on $T_C$. The same intuition
holds for $e_p$ entries as well; when a $e_c$ entry is checked for
dominance with $E_P$, first all leaf $e_p$ entries will be
examined. As long as there is no non-leaf $e_p$ that dominates $e_c$,
\rsl proceeds with expanding the nearest from $q$ non-leaf $e_p$
entry. This change in the visiting order of $E_P$ reduces the number
of accesses on $T_P$ as well.
}



%Before giving details on \rsl algorithm, we present two additional properties:

%\begin{property}
%If $c_i \in RSKY(q)$ and $c_j \prec_q c_i$, then $c_j \in RSKY(q)$
%\label{prop:lemma1}
%\end{property}
%\begin{property}
%If $c_i \not\in RSKY(q)$ and $c_i \prec_q c_j$, then $c_j \not\in RSKY(q)$
%\label{prop:lemma2}
%\end{property}

%Returning to Fig.~\ref{fig:region}, if $c_2$ does not belong to $RSKY(q)$, then $c_4$ will not belong to $RSKY(q)$ either. On the other hand, if $c_2$ belongs to $RSKY(q)$, then $c_5$ belongs to $RSKY(q)$ as well.


\stitle{Algorithm Description.}  Now, we describe the execution of
our \rsl algorithm, while providing its detailed
pseudocode in Alg.~\ref{alg:rsl}.\eat{ \rsl employs two indexes,
an R-tree $T_P$ on the set of products $P$ and another $T_C$ on the
set of customers $C$.}  Initially, \rsl inserts all root entries of
$T_P$ (resp. $T_C$) in the priority queue $E_P$ (resp. $E_C$).\eat{
sorted on $e_x$'s level and $e_x$ Euclidean distance \emph{mindist}
from $q$ as key, as explained above.} Further, \rsl maintains a set
$SKY(q)$ of the currently found midpoint skylines which are used for
pruning based on Lemma~\ref{lem:ir_rss}. \rsl proceeds in
iterations. In each iteration \rsl extracts the entry in $E_C$ having
the minimum key from $q$ (Line~5) and checks the following pruning
conditions:
\newcounter{Lcount49}
\begin{list}{\arabic{Lcount49}.}
  {
    \usecounter{Lcount49}
    \setlength{\labelwidth}{12pt}
    \setlength{\leftmargin}{0pt}
    \setlength{\itemindent}{\labelwidth}
    \setlength{\parskip}{1pt}
    \setlength{\parsep}{1pt}
    \setlength{\itemsep}{1pt}
  }

%\begin{enumerate}

\item If $e_c$ is dominated by any point that belongs in the currently
found midpoint skylines $SKY(q)$, $e_c$ can be removed from $E_C$
based on Lemma~\ref{lem:ir_rss} (Lines~6-8).

\item Otherwise, if $e_c$ is a non-leaf entry (Line~9), $e_c$ is
expanded and children nodes are inserted into $E_C$ (Line~10 and
Alg.~\ref{alg:IOaccess}, described later in this section).

\item Else, for all $e_p$ entries in $E_P$ (Lines~12-22):

\squishlist

\item If $e_c$ is dominated by the midpoint of a leaf entry $e_p \in
E_P$ (Line~15), then $e_c$ can be removed from $E_C$, based
on Lemma~\ref{lem:ir_rss}, and the midpoint of $e_p$ is inserted into
$SKY(q)$ (Line 17)).

\item Else if $e_c$ is dominated by the midpoint of the
\emph{min-corner} $e^-_{p}$ of a non-leaf $e_p \in E_P$, $e_p$ is
expanded and its children entries are inserted into $E_P$ (Line~21).

\squishend

\end{list}

Finally, if $e_c$ has not been pruned by any of the above conditions,
then $e_c$ is a reverse skyline point (Lines~23-24) and can be at that
stage directly reported in the result. The \rsl algorithm terminates
when $E_C$ becomes empty and then $RSKY(q)$ is returned
(Line~25).\eat{ Alg.~\ref{alg:rsl} provides the detailed pseudocode
for the \rsl algorithm.}


%\begin{figure}[t]
%\vspace{-5pt}
\begin{algorithm}[t]
\begin{scriptsize}
	\KwIn{$q$ a query point, $T_P$ R-tree on products, $T_C$ R-tree on customers, $E_P(q)$ priority queue on product entries, $E_C(q)$ priority queue on customer entries}
	\KwOut{$RSKY(q)$ reverse skylines of $q$}
	\SetKwInput{KwVar}{Variables}
	\KwVar{$SKY(q)$ currently found midpoint skylines of products w.r.t $q$}
	\Begin
	{
        $SKY(q) := \varnothing; RSKY(q) := \varnothing$\;
        \While{$E_C \neq \varnothing$}
        {
            dominated := false\;
            $E_C(q).pop() \rightarrow e_c$\;
            \If{dominated($e_c$, $SKY(q))$}
            {
                dominated := true\;
                continue\;
            }
            \If{$e_c$ is a non-leaf entry}
            {
                %\ForAll{$e_{c_l}$ children of $e_c$}
%                {
%                    \If{(dominated($e_{c_l}$, $SKY(q))$ == false)}
%                    {
%                        $E_C(q).push(e_{c_l})$\;
%                    }
%                }
                 EntryExpand($e_c$, $SKY(q)$, $E_C(q)$, $T_C$)\;
            }
            \Else
            {
                \ForEach{$e_p \in E_P(q)$}
                {
                    $midpoint(e_p, q) \rightarrow m$\;
                    \If{$e_c$ is dominated by $m$}
                    {
                        \If{$e_p$ is a leaf entry}
                        {
                            \If{(dominated($m$, $SKY(q))$ == false)}
                            {
                                $SKY(q).push(m)$\;
                            }
                            dominated := true\;
                            break\;
                        }
                        \Else
                        {
                            %\If{dominated($e_p$, $SKY(q))$}
%                            {
%                                $E_P(q).remove(e_p)$\;
%                            }
%                            \Else
%                            {
                            EntryExpand($e_p$, $SKY(q)$, $E_p(q)$, $T_P$)\;
%                            }
                        }
                        $E_P(q).remove(e_p)$\;
                    }
                }
                \If{(dominated == false)}
                {
                    $RSKY(q).push(e_c)$\;
                }
            }
	   }
    \Return{$RSKY(q)$}\;
    }
\caption{\rsl}
\label{alg:rsl}
\end{scriptsize}
	%\nocaptionofalgo
	%\label{fig:rsl}
\end{algorithm}
%\vspace{-10pt}
%\caption{RSL}
%\vspace{-10pt}
%\label{fig:rsl}
%\vspace{-5pt}
%\end{figure}


\stitle{Optimizations.} Observe that any product entry that is already dominated w.r.t. to $q$ by any currently found skyline point, will definitely not contribute in further refining the $RSKY(q)$. Consequently, it can be safely pruned from further processing. We apply this observation as an additional optimization step whenever expanding a product entry. The detailed pseudocode is provided in Alg.~\ref{alg:IOaccess}.

In particular, whenever a $e_p$ ($e_c$) entry is expanded, before inserting children nodes to $E_P$ ($E_C$), the \rsl algorithm performs the following: First a temporary queue is created and children nodes are iteratively pushed inside the queue (Line 8). When expanding a customer entry, each child node is checked only with the currently found $SKY(q)$ (Line 7). If it is dominated, then the child node can be pruned according to Lemma~\ref{lem:ir_rss}. On the other hand, when expanding a product entry $e_p$, before pushing $e_p$'s children nodes inside the temporary queue, each children node is checked for dominance w.r.t to $q$ with: (\emph{i}) children nodes already inside the queue (Line 5), and (\emph{ii}) the currently found $SKY(q)$ (Line 7). Finally, after all qualified children
nodes have been determined they are pushed inside $E_P$ ($E_C$) (Line 10).

This optimization results in fewer children nodes pushed inside the priority queues $E_P$ ($E_C$) which leads to: (\emph{i}) less space needed for $E_P$ ($E_C$) in intermediate iterations, and (\emph{ii}) reduced processing time for subsequent dominance checks, since reducing the number of pushed entries results in fewer entries being processed in the future and in smaller data structures being used.

%Essentially, instead of inserting entries individually, all remaining entries in the queue are bulk-loaded in a single operation. This reduces the time \textbf{{\large HOW? EXPLAIN IN DETAIL}} required to reorganize each priority queue during the insertion of children node entries. %Algorithm~\ref{alg:IOaccess} presents the pseudocode for these optimizations (Lines~3-8 and Line~9, respectively).

\begin{algorithm}[t]
\begin{scriptsize}
	\KwIn{$e_x$ a product or customer entry, $SKY(q)$ currently found midpoint skyline set w.r.t to $q$, $E_x(q)$ priority queue on $e_x$, $T_x$ index on $e_x$}
    \KwOut{$E_x(q)$}
	\SetKwInput{KwVar}{Variables}
	\KwVar{$L$ queue on children of $e_x$}
	\Begin
	{
        $L := \varnothing$\;
        \ForEach{$e_{x_l}$ children of $e_x$}
        {
            \If{$e_x$ is a product entry}
            {
                \If{(dominated($e_{x_l}$, $L$) == true)}
                {
                    continue;
                }
            }
            \If{(dominated($e_{x_l}$, $SKY(q)$) == false)}
            {
                $L.push(e_{x_l})$\;
            }
        }
        \ForEach{$e_{x_l} \in L$}
        {
            $E_x(q).push(e_{x_l})$\;
        }
        \Return{$E_x(q)$}\;
    }
\caption{EntryExpand}
\label{alg:IOaccess}
\end{scriptsize}
\end{algorithm}


